Linear Runlength-Limited Subcodes of Reed-Muller Codes and Coding Schemes for Input-Constrained BMS Channels

In this work, we address the question of the largest rate of linear subcodes of Reed-Muller (RM) codes, all of whose codewords respect a runlength-limited (RLL) constraint. Our interest is in the $(d,\infty)$-RLL constraint, which mandates that every pair of successive $1$s be separated by at least $d$ $0$s. Consider any sequence $\{{\mathcal{C}_m}\}_{m\geq 1}$ of RM codes with increasing blocklength, whose rates approach $R$, in the limit as the blocklength goes to infinity. We show that for any linear $(d,\infty)$-RLL subcode, $\hat{\mathcal{C}}_m$, of the code $\mathcal{C}_m$, it holds that the rate of $\hat{\mathcal{C}}_m$ is at most $\frac{R}{d+1}$, in the limit as the blocklength goes to infinity. We also consider scenarios where the coordinates of the RM codes are not ordered according to the standard lexicographic ordering, and derive rate upper bounds for linear $(d,\infty)$-RLL subcodes, in those cases as well. Next, for the setting of a $(d,\infty)$-RLL input-constrained binary memoryless symmetric (BMS) channel, we devise a new coding scheme, based on cosets of RM codes. Again, in the limit of blocklength going to infinity, this code outperforms any linear subcode of an RM code, in terms of rate, for low noise regimes of the channel.

==> BCJR_invar.tex <==
\label{subsec:BCJR_invar}

Given the $Q$-graph, $\mathscr{G}_Q^{(d)}$, for the $(d,\infty)$-RLL input constrained BEC, we call its corresponding $(S,Q)$ graph, $\mathscr{G}_{SQ}^{(d)}$, which is constructed following the description in definition \ref{def:SQ_graph}, with the presentation of channel states given in figure \ref{fig:d_inf_constraint}. 


%We note that our family of $(S,Q)$-graphs  possesses the following interesting property:
%
%\begin{proposition}\label{prop:lp}
%	In the setting of the $(d,\infty)$-RLL input-constrained BEC, for the $(S,Q)$-graphs, $\mathscr{G}_{SQ}^{(d)}$, we have that 
%	\begin{equation*}
%	\max_{\{{P}(x|s,v)\}} P(X=1)\leq \frac{1}{d+1},
%	\end{equation*}
%	where the maximum is taken over all input distributions, $\left({P}(\cdot|s,v): s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$ such that the resulting Markov chain on $\mathscr{S}\times \mathscr{V}^{(d)}$ has a unique stationary distribution.
%\end{proposition}
%
%We prove Proposition \ref{prop:lp} by casting the maximization problem as a linear program (LP). We then use the weak duality theorem for LPs (see, for example, \cite{boyd}) to find a feasible point of the corresponding dual LP, the objective value at which serves as an upper bound for our maximization problem. The proof is dealt with in Appendix C.

In this subsection, we construct a BCJR-invariant input distribution, $\left(\left(\tilde{P}(x|s,v):x\in \mathscr{X}\right): (s,v)\in \mathscr{S}\times \mathscr{V}^{(d)}\right)$. In tandem, we will also identify the conditional distribution, $\left(\tilde{\pi}(s|v):s\in \mathscr{S}\right)$, for each $v\in \mathscr{V}^{(d)}$, where $\left(\tilde{\pi}(s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$ is the stationary distribution on the nodes of $\mathscr{G}_{SQ}^{(d)}$
%, and $\tilde{\pi}(v) = \sum_{s\in \mathscr{S}}\tilde{\pi}(s,v)$.

%Before we do so, it will be useful to put down some additional notation. Now, for $\mathbf{q}\in \mathscr{V}^{(d)}$, let $(k_1^{\mathbf{q}},k_2^{\mathbf{q}},\ldots,k_{d+1}^{\mathbf{q}})$ denote the runlength sequence of $0$s and $?$s, in $\mathbf{q}$, defined as follows:

%If $\mathbf{q}$ begins with a run of $\ell$ $0$s, for $\ell \geq 1$, then $k_1^{\mathbf{q}} = \ell$; otherwise, $k_1^{\mathbf{q}} = 0$. Further, $k_2^{\mathbf{q}}$ is the length of the run of $?$s after the first run (if any) of $0$s; $k_3^{\mathbf{q}}$ is the length of the (second) run of $0$s after the first run of $?$s, and so on. 

%Note that $k_{2i-1}^{\mathbf{q}}$ records the length of a run of $0$s and $k_{2i}^{\mathbf{q}}$ records the length of a run of $?$s, for $i\geq 1$. Also, $k_{d+1}^{\mathbf{q}}\neq 0$ if, and only if, $\mathbf{q}$ is such that $q_{2i-1}=?$ and $q_{2i}=0$, for $i\geq 1$. Observe that $\sum_{i=1}^{d+1}k_i^{\mathbf{q}} = d$ and $k_i^{\mathbf{q}}\geq 0$, for all $i\in [d+1]$. We shall henceforth omit the superscript $\mathbf{q}$ since it will be apparent from the context.

Since our input distribution %$\left(\tilde{P}(\cdot|s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$,
must respect the $(d,\infty)$ input constraint, we need that $\tilde{P}(1|s,v)=0$, for $s\in \{0,1,\ldots,d-1\}$, and we hence need only specify $\tilde{P}(1|d,v)$, for each $v\in \mathscr{V}^{(d)}$, to completely determine the input distribution.

To this end, we first associate with every node $v\in \mathscr{V}^{(d)}$, a probability vector, $\boldsymbol{\theta}_v:=\left(\theta_v(s):s\in \mathscr{S}\right)$, of length $d+1$. 
%The vector $\boldsymbol{\theta}_v$ is a proxy for $\left(\tilde{\pi}(s|v):s\in \mathscr{S}\right)$ for a suitably defined input distribution.

We set $\boldsymbol{\theta}_{Q_i} = \mathbf{e}_{i}^{d}$, for $i\in [0:d]$. Further, in compliance with the $(d,\infty)$-RLL input constraint, we set $a_{Q_i}:=\tilde{P}(1|d,Q_i) = 0$, for $i\neq d$. Let us pick $a := \tilde{P}(1|d,Q_d)$, such that $a\leq \frac{1}{d+1}$. The reason for the restriction of $a$ to the interval $[0,\frac{1}{d+1}]$ will be made clear in Lemma \ref{lemma:domain}. 
%We shall, for conciseness of notation, represent $a_{Q_d}$ as $a$.

Now, for $\mathbf{q} = (w_{0},w_{1},\ldots,w_{d-1})\in \mathscr{V}^{(d)}_{\text{DB}}$, we define an accompanying vector $\boldsymbol{\beta}=(\beta_{0},\beta_{1},\ldots,\beta_{d-1})$, with\\ $\beta_s := |\{i\in [0:s-1]:w_i=0\}|$. In words, $\beta_s$ is the number of $0$s that appear strictly to the left of position $s$ in the $d$-tuple corresponding to $\mathbf{q}$. We then define $\boldsymbol{\theta}_{\mathbf{q}}$ as follows:

For $0\leq s\leq d-1$,
\begin{equation}\label{eq:theta_even}
{\theta}_{\mathbf{q}}(s) = 
\begin{cases}
0, & \text{ if } w_s=0,\\
\frac{a}{(1-a)^{\beta_s}}, & \text{ if }  w_s=\ ?,
\end{cases}
\end{equation}
and $\theta_{\mathbf{q}}(d) = 1-\sum_{s=0}^{d-1}\theta_{\mathbf{q}}(s)$. It is clear from our definition that $\boldsymbol{\theta}_{Q_d} = \mathbf{e}_{d}^{d}$, where $Q_d = (0,0,\ldots,0)\in \mathscr{V}_{\text{DB}}^{(d)}$.

%If $d$ is odd, for $\mathbf{q} \in \mathscr{V}_{\text{DB}}^{(d)}$, we set
%\begin{equation}\label{eq:theta_odd}
%\theta_{\mathbf{q}}(s) = 
%\begin{cases}
%a, \ s\in [0:k_{d+1}-1],\\
%0, \ s\in [k_{d+1}:k_{d+1}+k_d-1],\\
%\frac{a}{(\bar{a})^{k_d}}, \ s\in [k_{d+1}+k_d:\sum\limits_{i\geq {d-1}}k_i -1],\\
%0, \ s\in [\sum\limits_{i\geq {d-1}}k_i:\sum\limits_{i\geq {d-2}}k_i-1],\\
%\quad \vdots\\
%\frac{a}{(\bar{a})^{\sum\limits_{i\geq 3: i\ \text{odd}}k_i}}, \ s\in [\sum\limits_{i\geq {3}}k_i:\sum\limits_{i\geq {2}}k_i],\\
%0, \ s\in [\sum\limits_{i\geq {2}}k_i:d-1],
%\end{cases}
%\end{equation}
%and $\theta_{\mathbf{q}}(d) = 1-\sum_{i=1}^{d-1}\theta_{\mathbf{q}}(i)$.

Finally, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, we let $a_{\mathbf{q}}:= \tilde{P}(1|d,\mathbf{q}) = \frac{a}{\theta_{\mathbf{q}}(d)}$. In order for $a_{\mathbf{q}}$ to be a valid probability, it must lie in $[0,1]$, a sufficient condition for which is provided by Lemma \ref{lemma:domain} below.

\begin{lemma}\label{lemma:domain}
	For $a\in [0,\frac{1}{d+1}]$, $a_{\mathbf{q}}\in [0,1]$, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$ .
\end{lemma}

%The proof of this lemma is taken up in  Appendix A.
We refer the reader to \cite{fv} for the proof of the lemma above.
\begin{remark}
%Note that this procedure determines the vector $\left(a_v:v\in \mathscr{V}^{(d)}\right)$, thereby specifying the entire input distribution $\left(\tilde{P}(\cdot|s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$.

Our input distribution is aperiodic for $a<\frac{1}{d+1}$ and $\epsilon\neq 1$, as then there exists a self-loop of positive probability, $\bar{a}\bar{\epsilon}$, from the node $(d,Q_d)$ to itself, in $\mathscr{G}_{SQ}^{(d)}$. The feedback capacity at $\epsilon=1$ is well-known to be $C^{\text{fb}}(1) = 0$, and we safely assume, going forward, that $\epsilon\neq 1$.
\end{remark}

%\begin{figure*}[t]
%	\centering
%	\subfloat[]{\includegraphics[width=0.2\linewidth]{1_inf.png}\label{fig:Q_1}}
%	\hfill
%	\subfloat[]{\includegraphics[width=0.4\linewidth]{2_inf.png}\label{fig:Q_2}}
%	\caption{The $Q$-graphs $\mathscr{G}^{(1)}_Q$ and $\mathscr{G}^{(2)}_Q$ are shown above in (a) and (b), respectively. Note that the nodes in the de Bruijn components are labelled by $d$-tuples, with $Q_1 = 0$, in $\mathscr{G}^{(1)}_Q$, and $Q_2 = (0,0)$, in $\mathscr{G}^{(2)}_Q$. The parallel edges defined are here represented as a single edge with the label $(0,?)$, according to \eqref{eq:label}.}
%\end{figure*}
%\begin{figure}[t]
%	\centering
%	\includegraphics[scale=0.5]{2_inf_mod.png}
%	\caption{The $Q$-graph $\mathscr{G}^{(2)}_Q$ is shown above. Note that the nodes in the de Bruijn components are labelled by $d$-tuples, with $Q_2 = (0,0)$. The parallel edges defined are here represented as a single edge with the label $(0,?)$, according to \eqref{eq:label}.}
%	\label{fig:Q_2}
%\end{figure}
%Before we set out to prove that the aperiodic input distribution $\tilde{P}$ is indeed BCJR invariant, we shall introduce one other piece of notation. For the function $B_s: \Delta(d)\times \mathscr{Y} \rightarrow \Delta(d)$ defined in equation \eqref{eq:bs}, we define the vector $\mathbf{B}(\mathbf{\theta_v},y)$ to be $\left(B_s(\mathbf{\theta_v},y): s\in \mathscr{S}, s\neq d\right)$, for $v\in \mathscr{V}^{(d)}$. For the $(d,\infty)$-RLL input constrained BEC with the input distribution $\tilde{P}$, we can write down $\mathbf{B}(\mathbf{\theta_v},y)$ explicitly. For $v\in \mathscr{V}_{\text{DB}}^{(d)}$,

Before we prove that the aperiodic input distribution $\tilde{P}$ is indeed BCJR-invariant, we note that for all $s\in \mathscr{S}$ and $v\in \mathscr{V}^{(d)}$, the value $B_s(\boldsymbol{\theta}_v,y)$ (see equation \eqref{eq:bs}) can be computed explicitly for the $(d,\infty)$-RLL input constrained BEC with the input distribution $\tilde{P}$. 
%\begin{equation*}
%\mathbf{B}(\mathbf{\theta_v},y) = \begin{cases}
%\left[0,\frac{\theta_{\mathbf{q}}(0)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)},\frac{\theta_{\mathbf{q}}(1)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)},\ldots,\frac{\theta_{\mathbf{q}}(d-2)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)}\right], \ y=0,\\
%\left[a_\mathbf{q}\theta_{\mathbf{q}}(d),\theta_{\mathbf{q}}(0),\theta_{\mathbf{q}}(1),\ldots,\theta_{\mathbf{q}}(d-2)\right], \ y=?,\\
%[1,0,0,\ldots,0], \ y=1,
%\end{cases}
%\end{equation*}
%
For $0\leq s\leq d-1$, and for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, it holds that
\begin{equation}\label{eq:Bs0}
B_s(\boldsymbol{\theta}_\mathbf{q},y) = 
\begin{cases}
0, & \text{ if } s=0,\ y=0\\
\frac{\theta_{\mathbf{q}}(s-1)}{1-a_\mathbf{q}\theta_{\mathbf{q}}(d)} = \frac{\theta_{\mathbf{q}}(0)}{1-a}, & \text{ if } 1\leq s \leq d-1, \ y=0\\
a_\mathbf{q}\theta_{\mathbf{q}}(d) = a & \text{ if } s=0, \ y=?\\
\theta_{\mathbf{q}}(s-1), & \text{ if } 1\leq s \leq d-1, \ y=?\\
1, & \text{ if } s=0, \ y=1\\
0, & \text{ if } 1\leq s \leq d-1, \ y=1,
\end{cases}
\end{equation}
with $B_d(\boldsymbol{\theta}_\mathbf{q},y) = 1 - \sum_{s=0}^{d-1}B_s(\boldsymbol{\theta}_\mathbf{q},y)$, for $y\in \{0,?,1\}$. Note that the vector $\left(B_s(\boldsymbol{\theta}_\mathbf{q},1): s\in \mathscr{S}\right)$ is equal to $\mathbf{e}_0^{d}$.
%which results in
%\begin{equation}\label{eq:bs_BEC}
%\mathbf{B}(\mathbf{\theta_v},y) = 
%\begin{cases}
%\left[0,\frac{\theta_{\mathbf{q}}(0)}{1-a},\frac{\theta_{\mathbf{q}}(1)}{1-a},\ldots,\frac{\theta_{\mathbf{q}}(d-2)}{1-a}\right], \ y=0,\\
%\left[a,\theta_{\mathbf{q}}(0),\theta_{\mathbf{q}}(1),\ldots,\theta_{\mathbf{q}}(d-2)\right], \ y=?,\\
%[1,0,0,\ldots,0], \ y=1,
%\end{cases}
%\end{equation}
%since $a_\mathbf{q}\theta_{\mathbf{q}}(d)=a$.

Further, if $v=Q_i$, for some $i\in [0:d-1]$, it holds that
\begin{equation}\label{eq:BsQ}
\left(B_s(\boldsymbol{\theta}_v,y): s\in \mathscr{S}\right) = \mathbf{e}_{i+1}^{d},
\end{equation}
for $y\in \{0,?\}$.
%\begin{equation}\label{eq:bs_BEC_2}
%\mathbf{B}(\mathbf{\theta_v},y) = \mathbf{e}_{i+1}^{d},\ \text{for}\ y\in \{0,?\}.
%\end{equation} 
We now note that the following lemma holds:

\begin{lemma}\label{lemma:bcjr}
	The set of probability vectors $\left(\boldsymbol{\theta}_{v}: v\in \mathscr{V}^{(d)}\right)$ along with the input distribution $\left(\tilde{P}(\cdot|s,v):s\in \mathscr{S},\ v\in \mathscr{V}^{(d)}\right)$ satisfies
	\begin{equation}\label{eq:bs_valid}
	\theta_{v^+}(s^+) = B_{s^+}(\boldsymbol{\theta}_v,y),
	\end{equation}
	for every $(s^+,v,y)\in \mathscr{S}\times \mathscr{V}^{(d)}\times \mathscr{Y}$, where $v^+ = \Phi(v,y)$, with $\Phi:\mathscr{V}^{(d)}\times \mathscr{Y}\rightarrow \mathscr{V}^{(d)}$ is the $Q$-node update function.
\end{lemma}
\begin{proof}
	If $v=Q_i$, for some $i\in [0:d-1]$, then, it follows from equation \eqref{eq:BsQ} that 	
	$\mathbf{e}_{i+1}^{d}=\left(B_s(\boldsymbol{\theta}_{Q_i},y):s\in \mathscr{S}\right)
	$ which, in turn, is equal to  $\boldsymbol{\theta}_{Q_{i+1}}$,	
	for $y\in \{0,?\}$. Equation \eqref{eq:bs_valid} then follows by noting that $\Phi(Q_i,y) = Q_{i+1}$, for $y\in \{0,?\}$.
	
	Now, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, when $y=1$, we see from equation \eqref{eq:Bs0} that	
	$\mathbf{e}_{0}^{d}=\left(B_s(\boldsymbol{\theta}_{v},1):s\in \mathscr{S}\right)$, which is equal to $\boldsymbol{\theta}_{Q_{0}}$.
	Since $\Phi(v,1) = Q_{0}$, it follows that equation \eqref{eq:bs_valid} holds.
	
	Now, let $\mathbf{q} = (w_{0},w_{1},\ldots,w_{d-1})\in \mathscr{V}_{\text{DB}}^{(d)}$. Then, since $\Phi(\mathbf{q},0) = (0,w_{0},w_{1},\ldots,w_{d-1}))=:\mathbf{q}_0^+$, and $\Phi(\mathbf{q},?) = (?,w_{0},w_{1},\ldots,w_{d-1})=:\mathbf{q}_?^+$,  we see from equations \eqref{eq:theta_even} and \eqref{eq:Bs0} that $\left(B_s(\boldsymbol{\theta}_\mathbf{q},0):s\in\mathscr{S}\right) = \boldsymbol{\theta}_{\mathbf{q}^+_0}$ and $\left(B_s(\boldsymbol{\theta}_\mathbf{q},?):s\in\mathscr{S}\right) = \boldsymbol{\theta}_{\mathbf{q}^+_?}$. Thus, equation \eqref{eq:bs_valid} holds in this case too.	
\end{proof}
We now define the joint distribution, $\theta(s,v):=\theta_v(s)\tilde{\pi}(v)$, where $\left(\tilde{\pi}(v):v\in \mathscr{V}^{(d)}\right)$ is the stationary distribution on the nodes of $\mathscr{G}_Q^{(d)}$ induced by $\tilde{P}$. From Lemma \ref{lemma:bcjr} and from the lemma below, we get that $\tilde{P}$ is BCJR-invariant.

\begin{lemma}\label{lemma:stat_dist}
	It holds that $\theta(s,v) = \tilde{\pi}(s,v)$, for all $s\in \mathscr{S}$ and $v\in \mathscr{V}^{(d)}$.
\end{lemma}
\begin{proof}
	Fix an $s^+ \in \mathscr{S}$, and a $v^{+}\in \mathscr{V}^{(d)}$. Now,
	\begin{align*}
	&\sum\limits_{s,v,x,y}\theta(s,v)P(x|s,v)P(y|x)\mathds{1}\{s^+=f(x,s)\}\mathds{1}\{v^+=\Phi(v,y)\}\\
	&= \sum\limits_{v,y}\tilde{\pi}(v)\mathds{1}\{v^+=\Phi(v,y)\}\sum\limits_{x,s}\theta_v(s)P(x|s,v)P(y|x)\times\\
	&\quad \quad \quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad\quad \mathds{1}\{s^+=f(x,s)\}\\
	&\stackrel{(a)}{=}\theta_{v^+}(s^+)\sum\limits_{v,y}\tilde{\pi}(v)P(y|v)\mathds{1}\{v^+=\Phi(v,y)\}\\
	&=\theta_{v^+}(s^+)\tilde{\pi}(v^+) = \theta(s^+,v^+),
	\end{align*}
	where (a) follows from Lemma \ref{lemma:bcjr}, since $\theta_{v^+}(s^+)P(y|q)=\sum\limits_{x,s}\theta_v(s)P(x|s,v)P(y|x)\mathds{1}\{s^+=f(x,s)\}$. Since this holds for all $(s^+,v^+) \in \mathscr{S}\times \mathscr{Y}$, it follows that $\theta(s^+,v^+) = \tilde{\pi}(s^+,v^+)$.
\end{proof}
The lemma above implies that $\boldsymbol{\theta}_v = \tilde{\pi}(\cdot|v)$, and using Lemma \ref{lemma:bcjr}, we can conclude that $\tilde{P}$ is BCJR-invariant.
\begin{remark}
	It can be shown that for a fixed value of $a$, there is a unique BCJR-invariant input distribution on $\mathscr{G}_{SQ}^{(d)}$. 
	%In particular, this means that for a fixed value of $a$, the probability\\ $P(Y=1|\mathbf{q}) = a\epsilon$, for all $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$.
\end{remark}

==> Proof_UB.tex <==
\label{sec:proof_UB}
\begin{proof}
We shall compute the upper bound expression in theorem \ref{thm:UB} by considering the family of $Q$-graphs, $\mathcal{J}:=\{\hat{\mathscr{G}}_Q^{(d)}: d\in \mathbb{N}\}$, where $\hat{\mathscr{G}}_Q^{(d)}$ is shown in figure \ref{fig:G_hat} for some fixed $d$. Let $\hat{\mathscr{G}}_{SQ}^{(d)}$ denote the $(S,Q)$-graph corresponding to $\hat{\mathscr{G}}_Q^{(d)}$. 

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.5\textwidth]{UB_Q.png}
	\caption{The $Q$-graph, $\hat{\mathscr{G}}_Q^{(d)}$. The labels on the edges denote outputs.}
	\label{fig:G_hat}
\end{figure*}

It can be shown that the single closed communicating class in $\hat{\mathscr{G}}_{SQ}^{(d)}$ is precisely the collection $\{(i,\hat{Q}_i): i\in [0:d-1]\}\cup \{(s,\hat{Q}_d):s\in [0:d]\}$ of nodes. Further, since the inputs are constrained, it holds that $P(X=1|S=s,Q=\hat{q}) = 0$, for all $(s,\hat{q}) \neq (d,\hat{Q}_d)$, with $(s,\hat{q})$ in the closed class. Therefore, the matrix of conditional input distributions, $[P(x|s,\hat{q})]$, can be parameterized by a single parameter, $p:=P(X=1|S=d,Q=\hat{Q}_d)$.

A simple computation then reveals that the stationary distribution of nodes in the closed communicating class obey:
\begin{align*}
\pi(s,\hat{Q}_s) &= \frac{p\bar{\epsilon}}{1+dp}, \ s\in [0:d-1],\\
\pi(s,\hat{Q}_d) &= \frac{p\epsilon}{1+dp}, \ s\in [0:d-1], \\
\pi(d,\hat{Q}_d) &= \frac{1}{1+dp}.
\end{align*}
Further, it holds that the conditional probability,

\begin{align*}
P(Y=1|\hat{Q}_d) &= P(Y=1,X=1,S=d|\hat{Q}_d)\\
&=p\bar{\epsilon}\frac{\pi(d,\hat{Q}_d)}{\sum_{s=0}^{d}\pi(s,\hat{Q}_d)}\\
&= \frac{p\bar{\epsilon}}{1+dp\epsilon}.
\end{align*}

Then, by Theorem \ref{thm:UB}, it holds that
\begin{align*}
C_{(d,\infty)}^{\text{fb}} &\leq \sup_{P(x|s,q)\in \Omega} I(X;Y|Q)\\
&= \sup_{P(x|s,q)\in \Omega} H(Y|Q) - h_b(\epsilon)\\
&\stackrel{(a)}{=} \max_{p\in [0,1]} \bar{\epsilon}\left(\sum_{s=0}^{d}\pi(s,\hat{Q}_d)\right)h_b\left(\frac{p}{1+dp\epsilon}\right)\\
&= \max_{p\in [0,1]} \frac{\bar{\epsilon}(1+dp\epsilon)}{1+dp}h_b\left(\frac{p}{1+dp\epsilon}\right)\\
&\stackrel{(b)}{=} \max_{\delta \in [0,\frac{1}{1+d\epsilon}]} R(\delta),
\end{align*}
where, in (a), we have used the identity that $H(a\bar{c},\bar{a}\bar{c},c) = h_b(c)+\bar{c}h_b(a)$, for all $a,c \in [0,1]$, and (b) follows by changing the variable used in the maximization to $\delta:= \frac{p}{1+dp\epsilon}$.

Now, we note that if $\epsilon^{\star}$ satisfies the equation
\[
(d\epsilon)^{\left(\frac{1}{1-\epsilon}+d\right)} = (1+d\epsilon)^d,
\]
then, the derivative evaluated at $\frac{1}{1+d\epsilon^{\star}}$,  $R^{\prime}\left(\frac{1}{1+d\epsilon^{\star}}\right)$, is equal to $0$. Further, from the proof of Corollaries \ref{coroll} in Appendix B, we observe that $R^{\prime}(\delta)$ is strictly decreasing in $\delta$, for $\delta\in [0,1]$. Hence, it follows that for $\epsilon>\epsilon^{\star}$, the derivative, $R^{\prime}\left(\frac{1}{1+d\epsilon}\right)>0$, with $R^{\prime}(0^+)>0$. 

Therefore, the non-causal capacity, which is a maximum over $[0,1]$ of $R(\delta)$, is strictly larger than the upper bound in Proposition \ref{lemma:UB}, for $\epsilon>\epsilon^{\star}$.
\end{proof}

==> Proof_main.tex <==
\label{sec:proof_thm}

\begin{proof}
For the $(d,\infty)$-RLL input-constrained BEC under the BCJR-invariant input distribution $\tilde{P}$ defined in subsection \ref{subsec:BCJR_invar}, we have that
\begin{align*}
I(X;Y|Q) &\stackrel{(a)}{=} H(Y|Q) - h_b(\epsilon)\\
&\stackrel{(b)}{=} \bar{\epsilon}\sum_{v\in \mathscr{V}^{(d)}}\tilde{\pi}(v)h_b(P(X=1|v)) + h_b(\epsilon)- h_b(\epsilon)\\
&\stackrel{(c)}{=} \bar{\epsilon}\sum_{\mathbf{q}\in \mathscr{V}^{(d)}_{\text{DB}}}\tilde{\pi}(\mathbf{q})h_b(P(X=1|\mathbf{q}))\\
&\stackrel{(d)}{=}\bar{\epsilon}h_b(a)\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}).
\end{align*}
where (a) follows from the fact that $H(Y|X,Q) = H(Y|X) = h_b(\epsilon)$, and (b) from the fact that $P(Y=?|v) = \epsilon$, for all $v\in \mathscr{V}^{(d)}$, with $P(Y=1|v) = \bar{\epsilon}P(X=1|v)$. We additionally use  the identity that $H(a\bar{c},\bar{a}\bar{c},c) = h_b(c)+\bar{c}h_b(a)$, for all $a,c \in [0,1]$. Further, (c) holds since $P(X=1|Q_i) = 0$, for $i\in [0:d-1]$. To obtain the equality (d), note that for any $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, $P(X=1|\mathbf{q}) = \tilde{\pi}(d|\mathbf{q})a_\mathbf{q}$. Hence, from Lemma \ref{lemma:stat_dist}, it follows that that $P(X=1|\mathbf{q}) = a$.

%Now, since for any $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, $P(X=1|\mathbf{q}) = \tilde{\pi}(d|\mathbf{q})a_\mathbf{q}$, we get from Lemma \ref{lemma:stat_dist} that $P(X=1|\mathbf{q}) = a$. Hence, it follows that
%
%\begin{equation}\label{eq:I_eval}
%I(X;Y|Q) = \bar{\epsilon}h_b(a)\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}).
%\end{equation}
Further, it is true that
\begin{align}\label{eq:stat_q}
1 &= \sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}) + \sum_{i=0}^{d-1}\tilde{\pi}(Q_i) \notag\\
&= \sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}) + d\tilde{\pi}(Q_0) \notag\\
&= (1+da\bar{\epsilon})\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q}),
\end{align}
where the penultimate equality holds since $\tilde{\pi}(Q_0) = \tilde{\pi}(Q_i)$, for all $i\in [d-1]$. The last equality follows from the observation that $\tilde{\pi}(Q_0) = \sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q})P(Y=1|\mathbf{q}) = \bar{\epsilon}a\sum_{\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}}\tilde{\pi}(\mathbf{q})$.

Plugging \eqref{eq:stat_q} back into equation (d), we obtain that $I(X;Y|Q) = \frac{h_b(a)}{da+\frac{1}{1-\epsilon}}$, and taking a maximum over all \\$a\in [0,\frac{1}{d+1}]$, we get the required result.
\end{proof}



==> Q-construction.tex <==
\label{sec:Q_const}
%We shall henceforth consider $\mathscr{S} = \{0,1,\ldots,d\}$ to be the state alphabet, for the $(d,\infty)$-RLL input constrained BEC.
%
%
In this section, we shall construct a family of $Q$-graphs, indexed by $d$, and identify a BCJR-invariant input distribution on the $(S,Q)$-graph corresponding to each $Q$-graph in the family.

\subsection{Construction of Q-graphs}
\input{Q-graph_fly.tex}

\subsection{Construction of a BCJR-invariant input distribution}
\input{BCJR_invar.tex}

==> Q-graph_fly.tex <==
%First, we recall the definition of a De Bruijn graph.
%
%\begin{definition}
%	Given an alphabet $\Sigma = \{w_1,w_2,\ldots,w_m\}$, a $k$-dimensional De Bruijn graph $\mathscr{G}_{\text{DB}}^{(k)} = (\mathscr{V}_{\text{DB}}^{(k)},\mathscr{E}_{\text{DB}}^{(k)},\mathscr{L}_{\text{DB}}^{(k)})$ over $\Sigma$ is a labelled, directed graph with vertex set $\mathscr{V}_{\text{DB}}^{(k)}$, edge set $\mathscr{E}_{\text{DB}}^{(k)}$, and a labelling function $\mathscr{L}_{\text{DB}}^{(k)}: \mathscr{E}_{\text{DB}}^{(k)}\rightarrow \Sigma$. Each vertex $v\in \mathscr{V}$ can be uniquely identified by a $k$-tuple over $\Sigma$, i.e., each vertex in $\mathscr{V}_{\text{DB}}^{(k)}$ can alternatively be written as $\mathbf{v} = (w_1^v,w_2^v,\ldots,w_k^v)$, where $w^v_i \in \Sigma$, for $i\in [k]$. Note that there are $m^k$ vertices in total.
%	
%	The edge set 	
%	\begin{align*}
%	\mathscr{E}_{\text{DB}}^{(k)} = \lbrace\mathbf{e}:\mathbf{e} = &\left((w_1^i,w_2^i\ldots,w_k^i),(w_2^i,w_3^i,\ldots,w_k^i,w)\right),\\
%	& \text{ for some $w_1^i,\ldots,w_k^i,w \in \Sigma$}\rbrace.
%	\end{align*}
%	
%	Further, for any edge \\$\mathbf{e} = \left((w_1^i,w_2^i\ldots,w_k^i),(w_2^i,w_3^i,\ldots,w_k^i,w)\right)$, we write \\ $\mathscr{L}(\mathbf{e}) = w$.
%\end{definition}
With each value of $d$ corresponding to the $(d,\infty)$-RLL input-constrained BEC, we associate a $Q$-graph, $\mathscr{G}_{Q}^{(d)} = (\mathscr{V}^{(d)},\mathscr{E}^{(d)},\mathscr{L}^{(d)})$, with vertex set $\mathscr{V}^{(d)}$, edge multi-set $\mathscr{E}^{(d)}$, and a labelling function $\mathscr{L}^{(d)}: \mathscr{E}^{(d)}\rightarrow \{0,?,1\}$.

We write $\mathscr{V}^{(d)} = \mathscr{V}_{\text{DB}}^{(d)} \cup \{Q_0, Q_1,\ldots,Q_{d-1}\}$, where each vertex in $\mathscr{V}_{\text{DB}}^{(d)}$ is uniquely identified by a $d$-tuple over $\{0,?\}$, i.e., each vertex in $\mathscr{V}_{\text{DB}}^{(d)}$ can be written as $\mathbf{q} = (w_{0}^q,w_{1}^q,\ldots,w_{d-1}^q)$, where $w^q_i \in \{0,?\}$, for $i\in \{0,1,\ldots,d-1\}$. In what follows, we suppress the superscript $q$, as it will be clear from the context. Note that there are $2^d$ vertices in $\mathscr{V}_{\text{DB}}^{(d)}$. We denote by $Q_d$, the vertex $(0,0,\ldots,0)\in \mathscr{V}_{\text{DB}}^{(d)}$.\footnote{The subscript ``DB'' indicates that the subgraph $\mathscr{G}_{\text{DB}}^{(d)} = (\mathscr{V}_{\text{DB}}^{(d)},\mathscr{E}_{\text{DB}}^{(d)},\mathscr{L}_{\text{DB}}^{(d)})$, of $\mathscr{G}_{Q}^{(d)}$, is a de Bruijn graph of order $d$, on $\{0,?\}$ symbols.}


We now construct the edge multi-set, $\mathscr{E}^{(d)}$. Firstly, for vertices in $\mathscr{V}_{\text{DB}}^{(d)}$, we define the set $\mathscr{E}_{\text{DB}}^{(d)}$ to consist of all edges $\mathbf{e} = \left((w_{0},w_{1}\ldots,w_{d-1}),(w,w_{0},w_1,\ldots,w_{d-2})\right)$, for $(w_{0},w_1\ldots,w_{d-1}), \ (w,w_{0},\ldots,w_{d-2}) \in \mathscr{V}_{\text{DB}}^{(d)}$. 
%\begin{align*}
%	\mathscr{E}_{\text{DB}}^{(d)} = & \lbrace\mathbf{e}:\mathbf{e} = \left((w_{0},w_{1}\ldots,w_{d-1}),(w,w_{0},w_1,\ldots,w_{d-2})\right),\\
%	& \ \ \ \ \ \text{ for }(w_{0},w_1\ldots,w_{d-1}), \ (w,w_{0},\ldots,w_{d-2}) \in \mathscr{V}_{\text{DB}}^{(d)} \rbrace.
%\end{align*}
%
Further, for any edge $\mathbf{e} = \bigl((w_{0},w_{1}\ldots,w_{d-1})$, $(w,w_{0},w_{1},\ldots,w_{d-2})\bigr)$, we define the labelling function $\mathscr{L}_{\text{DB}}^{(d)}: \mathscr{E}_{\text{DB}}^{(d)}\rightarrow \{0,?\}$ such that $\mathscr{L}_{\text{DB}}^{(d)}(\mathbf{e}) = w$.

%In this discussion, we shall focus on $d$-dimensional De Bruijn graphs, $\mathscr{G}_{\text{DB}}^{(d)}$, over $\Sigma = \{0,?\}$. By the definition above, this is a graph with $2^d$ vertices, each identified by a unique $d$-tuple consisting of $0,?$ symbols. Let us denote by $Q_d$, the vertex $(0,0,\ldots,0)\in \mathscr{V}_{\text{DB}}^{(d)}$.

%We construct the $Q$-graph, $\mathscr{G}_Q^{(d)} = (\mathscr{V}^{(d)},\mathscr{E}^{(d)},\mathscr{L}^{(d)})$, where $\mathscr{E}^{(d)}$ is now taken to be a multi-set, by first adding $d$ additional vertices, $Q_0,Q_1,\ldots, Q_{d-1}$, to $\mathscr{V}_{\text{DB}}^{(d)}$. Hence, $\mathscr{V}^{(d)} = \mathscr{V}_{\text{DB}}^{(d)} \cup \{Q_0,\ldots,Q_{d-1}\}$.

The edge set, $\mathscr{E}^{(d)}$, is constructed by adding to the set $\mathscr{E}_{\text{DB}}^{(d)}$, the edges $(\mathbf{q},Q_0)$, for $\mathbf{q}\in \mathscr{V}_{\text{DB}}^{(d)}$, and, corresponding to each $Q_i$, $i\in [0:d-1]$, two edges, $\mathbf{e}^{Q_i}_1$ and $\mathbf{e}^{Q_i}_2$, from $Q_i$ to $Q_{i+1}$. %Note that the $Q$-graph, $\mathscr{G}_Q^{(d)}$, has parallel edges. %which are precisely the edges from $Q_i$ to $Q_{i+1}$, for $i\in [0:d-1]$.

%\begin{figure*}[t]
%	\centering
%	\includegraphics[width=0.7\textwidth]{3_inf_LB_UB.png}
%	\caption{Plot comparing our lower bound with numerical evaluations of the upper bound from \cite{Graph_based}, for $d=3$.}
%	\label{fig:3_inf_compare}
%\end{figure*}



Finally, the labelling function, $\mathscr{L}^{(d)}:\mathscr{E}^{(d)}\rightarrow \{0,?,1\}$ is defined as:
\begin{equation}\label{eq:label}
\mathscr{L}^{(d)}(\mathbf{e})=
\begin{cases}
\mathscr{L}^{(d)}_{\text{DB}}(\mathbf{e}), & \text{ if } \mathbf{e}\in \mathscr{E}^{(d)}_{\text{DB}},\\
1, & \text{ if } \mathbf{e}=(\mathbf{q},Q_0) \text{ for } \mathbf{q}\in \mathscr{V}^{(d)}_{\text{DB}},\\
0 & \text{ if } \mathbf{e} = \mathbf{e}^{Q_i}_1 \text{ for some } i\in [0:d-1],\\
? & \text{ if } \mathbf{e} = \mathbf{e}^{Q_i}_2 \text{ for some } i\in [0:d-1].
\end{cases}
\end{equation}

%We note that $\mathscr{G}_Q^{(d)}$ satsifies the properties of a $Q$-graph detailed out in Section \ref{sec:Q-graph}. 
The $Q$-graph, $\mathscr{G}^{(1)}_Q$, is identical to the dynamic programming state diagram under the optimal policy, for the $(1,\infty)$-RLL input-constrained BEC \cite{SabBEC}. The $Q$-graph, $\mathscr{G}^{(2)}_Q$, is shown in Figure \ref{fig:Q_2}.

Our family of $Q$-graphs is then given by $\mathscr{H}:=\{\mathscr{G}^{(d)}_Q: d\in \mathbb{N}\}$, with the $Q$-graph $\mathscr{G}^{({d})}_Q$ being used to derive a lower bound for the $({d},\infty)$-RLL input-constrained BEC.
	
%\begin{remark}
%	The nodes $Q_0, Q_1,\ldots, Q_d$ of $\mathscr{G}^{(d)}_Q$ can be interpreted as follows. Let us define, for a fixed output sequence, $y^t$, the length-$(d+1)$ belief vector $\mathbf{z}_t:=\left(P(S_t=s_t|y^t):s_t\in \mathscr{S}\right)$. Note that the vector,  $\mathbf{z}_t$, which is an element of $\Delta(d)$, is precisely the state vector of the dynamic programming (DP) formulation of the feedback capacity problem \cite{Weiss}. The node $Q_i$ corresponds to the DP state $\mathbf{z}_t = \mathbf{e}_{i}^{d}$, for $i\in [0:d]$. This, in turn, has the interpretation that the nodes $Q_0,\ldots, Q_d$ represent the belief vectors when the decoder knows the channel state exactly.
%	
%%	Now, consider a node $\mathbf{q}\in \mathscr{V}^{(d)}_{\text{DB}}$, where $\mathbf{q}\in \{0,1\}^d$. Let $i_1,\ldots,i_k$, for $k\leq d$, denote the positions of the $?$ entries in in $\mathbf{q}$. We then interpret $\mathbf{q}$ as a proxy for the belief vector, $\mathbf{z}_t$, with non-zero entries in only the co-ordinates $d+1,d+1-i_1,\ldots,d+1-i_k$. Note that by our interpretation, $Q_d$, which represents the $d$-tuple $(0,\ldots,0)\in \mathscr{V}^{(d)}_{\text{DB}}$, corresponds to the belief vector $\mathbf{e}_{d+1}^{d+1}$, as described in the previous paragraph.
%\end{remark}




==> appA.tex <==
In this section, we show that the inequality $\beta(m)\leq \theta(m)$ holds, for large $m$ and sufficiently small $\delta>0$, with $\beta(m)$ and $\theta(m)$ defined in equations \eqref{eq:beta} and \eqref{eq:inter}, respectively. We fix an $R\in (0,R^*)$, where $R^*$ is defined in Theorem \ref{thm:rmub}.

We start with the expression 
\begin{equation}
\beta(m) = 2^{o(2^m)} \cdot \sum_{i=1}^{r_m-1} \exp_2 \left(\ln \left(\frac{1}{1-R}\right)\cdot 2^{m-i} - {m-2-i \choose \leq r_m}\right)
\label{eq:beta:2}
\end{equation}
We will split the sum $\sum\limits_{i=1}^{r_m-1}$ into two parts: $\sum\limits_{i=1}^{t_m}$ and $\sum\limits_{i={t_m}+1}^{r_m-1}$, where $t_m := \lfloor m^{1/3} \rfloor$.  For $i \in [t_m+1:r_m-1]$, we have
$$
\ln \left(\frac{1}{1-R}\right) \cdot 2^{m-i} - {m-2-i \choose \leq r_m} \ \le \  \ln \left(\frac{1}{1-R}\right) \cdot 2^{m-t_m} \ = \ o(2^m).
$$
Thus, the contribution of each term of the sum $\sum\limits_{i={t_m}+1}^{r_m-1}$ is $2^{o(2^m)}$, and since there are at most $r_m = O(m)$ terms in the sum, the total contribution from the sum is $2^{o(2^m)}$. 

Turning our attention to $i \in [t_m]$, we write
\begin{align}
\ln & \left(\frac{1}{1-R}\right) \cdot 2^{m-i} - {m-2-i \choose \leq r_m} \notag \\ & \ \ \ \ = \ 2^{m-2-i} \cdot \left[ 4 \ln\left(\frac{1}{1-R}\right) - \frac{1}{2^{m-2-i}} {m-2-i \choose \leq r_m}\right]. \label{i_in_tm_ineq}
\end{align}
By Lemma~\ref{lem:rate}, we obtain that $\frac{1}{2^{m-2-i}} {m-2-i \choose \leq r_m}$ converges to $R$ for all $i \in [t_m]$. In fact, with a bit more effort, we can show that this convergence is uniform in $i$. 
Note that, since $i \le t_m$, by virtue of \eqref{eq:rm_diff}, we have $|r_m - r_{m-2-i}|  \le  \frac{t_m+2}{2} + \frac{\sqrt{t_m+2}}{2} \lvert Q^{-1}(1-R)\rvert + 1 =: \nu_m$. Using the notation in the proof of Lemma~\ref{lem:rate}, we have $\frac{1}{2^{m-2-i}} {m-2-i \choose \leq r_m} = \Pr[S_{m-2-i} \le r_m]$. Thus, analogous to \eqref{sandwich}, we have for all sufficiently large $m$,
\begin{align*}
& \Pr[\overline{S}_{m-2-i} \le Q^{-1}(1-R) - \frac{\nu_m}{\frac12 \sqrt{m-2-t_m}}] \\
& \ \ \ \ \ \le \ \Pr[S_{m-2-i} \le r_m]  \\
& \ \ \ \ \ \ \ \ \ \ \ \le \ \Pr[\overline{S}_{m-2-i} \le Q^{-1}(1-R) + \frac{\nu_m}{\frac12 \sqrt{m-2-t_m}}].
\end{align*}
Now, we apply the Berry-Esseen theorem (see e.g., \cite[Theorem~3.4.17]{durrett}) which, in this case, asserts that $\left\lvert\Pr[\overline{S}_m \le x] - \Pr[Z \le x]\right\rvert \le 3/\sqrt{m}$, for all $x \in \mathbb{R}$ and positive integers $m$, where $Z \sim N(0,1)$. Thus, $\left\lvert\Pr[\overline{S}_{m-2-i} \le x] - \Pr[Z \le x]\right\rvert \le \frac{3}{\sqrt{m-2-i}} \le \frac{3}{\sqrt{m-2-t_m}}$ holds for all $x \in \mathbb{R}$ and $i \in [t_m]$. This yields
\begin{align*}
& \Pr[Z \le Q^{-1}(1-R) - \frac{\nu_m}{\frac12 \sqrt{m-2-t_m}}] - \frac{3}{\sqrt{m-2-t_m}} \\
& \ \ \le \ \Pr[S_{m-2-i} \le r_m]  \\
& \ \ \ \ \le \ \Pr[Z \le Q^{-1}(1-R) + \frac{\nu_m}{\frac12 \sqrt{m-2-t_m}}] + \frac{3}{\sqrt{m-2-t_m}}.
\end{align*}
Since $t_m$ and $\nu_m$ are both $o(\!\!\sqrt{m})$, we deduce that, as $m \to \infty$, $\Pr[S_{m-2-i} \le r_m] = \frac{1}{2^{m-2-i}} {m-2-i \choose \leq r_m}$ converges to $R$ uniformly in $i \in [t_m]$. 

Hence, for any $\delta \in (0,1)$ and $m$ large enough, it holds for all $i \in [t_m]$ that
\[
\frac{1}{2^{m-2-i}} {m-2-i \choose \leq r_m} \geq (1 - \delta) R,
\]
so that, carrying on from \eqref{i_in_tm_ineq}, 
$$
\ln \left(\frac{1}{1-R}\right) \cdot 2^{m-i} - {m-2-i \choose \leq r_m} \ \le \ 2^{m-3} \cdot \left[ 4 \ln\left(\frac{1}{1-R}\right) - (1-\delta)R \right]. \label{tm_ineq}
$$

To put it all together, recall that we split the sum $\sum\limits_{i=1}^{r_m-1}$ in \eqref{eq:beta:2} into two parts: $\sum\limits_{i=1}^{t_m}$ and $\sum\limits_{i={t_m}+1}^{r_m-1}$, where $t_m := \lfloor m^{1/3} \rfloor$. For sufficiently small $\delta > 0$, and all sufficiently large $m$, the contribution from the first sum is at most 
$$
m^{1/3} \cdot \exp_2\left(2^{m-3} \cdot \left[ 4 \ln\left(\frac{1}{1-R}\right) - (1-\delta)R \right] \right), 
$$
while that from the second sum is $\exp_2(o(2^m))$. Therefore, the overall sum $\sum\limits_{i=1}^{r_m-1}$ in \eqref{eq:beta:2} can be bounded above, for all sufficiently large $m$, by 
$$
2 m^{1/3} \cdot \exp_2\left(2^{m-3} \cdot \left[ 4 \ln\left(\frac{1}{1-R}\right) - (1-\delta)R \right] \right),
$$
Consequently,
$$
\beta(m) \ \le \ 2^{o(2^m)} \cdot \exp_2\Bigg( 2^{m-3}\Bigg[4\ln\left(\frac{1}{1-R}\right)  - R(1-\delta)\Bigg]\Bigg) \ =: \ \theta(m).
$$

==> fbcode.tex <==
\label{sec:fbcode}
This section presents a simple feedback coding scheme that achieves the lower bound in Theorem \ref{thm:main}. Our labelling-based coding scheme is similar to the coding schemes in \cite{SabBEC} and \cite{0k}. The main feature of the scheme is a dynamically-changing set of possible messages that is known to both the encoder and the decoder at all times. The objective of the encoder is to communicate a sequence of bits that will enable the decoder to narrow down the set of possible messages to a single message.

Each message $m\in [2^{nR}]$ is mapped uniformly to a point in the unit interval, i.e., the message $m$ is mapped to the point $\frac{m-1}{2^{nR}}$. At each time instant $i$, the unit interval is partitioned into sub-intervals that are labelled by either a `$0$' or a `$1$'. The input $x_i$ to the channel is determined using the label of the sub-interval containing the message. 

The coding scheme proceeds as follows: we first pick positive real numbers $\delta_0,\delta_1,\ldots,\delta_d$ such that $\sum\delta_i\leq 1$. To determine the input bits to be sent, we use a set of $d+2$ labellings, $\mathcal{L}_0,\ldots, \mathcal{L}_d,\hat{\mathcal{L}}$, with the interval $[\sum_{j<i}\delta_j,\sum_{j\leq i}\delta_j)$, in $\mathcal{L}_i$, labelled by a `$1$'. Further, labelling $\hat{\mathcal{L}}$ is such that the entire interval $[0,1)$ is labelled by a `$0$'. Figure \ref{fig:labellings} shows an illustration of the set of labellings.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.6\textwidth]{Labellings_new}
	\caption{The set of labellings, $\mathcal{L}_0,\ldots, \mathcal{L}_d$, used in the coding scheme.}
	\label{fig:labellings}
\end{figure}




\begin{algorithm}[t]
	\caption{Coding Scheme}
	\label{alg}
	\begin{algorithmic}[1]		
		\Procedure{Code}{m}       
		\State Set $\mathcal{M}_0 = [2^{nR}]$ and $Y_{1-d}^{0} = (0,\ldots,0)$.
		\State Set Label = $\mathcal{L}_0$.
		\State Set time index $i = 1$.
		\While{$|\mathcal{M}_{i-1}|>1$}
		\State Transmit $X_i = \Gamma(m,\text{Label})$. \Comment{Encoder}
		\If{none of $Y_{i-d}^{i-1}$ is a $1$}
		\If{$Y_i = 0$}
		\State Set $\mathcal{M}_i = \mathcal{M}_{i-1}^{(0)}$.
		\ElsIf{$Y_i=1$}
		\State Set $\mathcal{M}_i =\mathcal{M}_{i-1}^{(1)}$. 
		\Else
		\State Set $\mathcal{M}_i =\mathcal{M}_{i-1}$. 
		\EndIf
		\Else
		\State Set $\mathcal{M}_i =\mathcal{M}_{i-1}$. 
		\EndIf
		\State Label $\leftarrow$ $G(\text{Label},Y_{i-d+1}^{i})$.
		\State Update $i = i+1$.
		\EndWhile
		\State Output $\hat{m}$, where $\mathcal{M}_{i-1} = \{\hat{m}\}$. \Comment{Decoder}
		\EndProcedure
		
	\end{algorithmic}
\end{algorithm} 
The labelling at any time is a function of the channel outputs upto that time instant and can be recursively computed using the previous labelling and previous $d$ channel outputs. Thus, both the encoder and the decoder can compute the labelling used at all times. Let $L_i$ denote the labelling used at time $i$. We fix $L_0 := \mathcal{L}_0$. Then, $L_{i+1} = G(L_i,Y^{i}_{i-d+1})$, where the function $G$ is defined as follows:

\[G(L_i,Y^{i}_{i-d+1}) =
\begin{cases}
	\hat{\mathcal{L}},\ \text{ if one of $Y_{i-d+1}^{i}$ is a 1},\\
	\mathcal{L}_0,\ \text{if $Y_i=0$},\text{ and none} \text{ of $Y_{i-d+1}^{i}$ is a 1},\\
	\mathcal{L}_{\text{$j+1$ mod$(d+1)$}},\ \text{if $L_i = \mathcal{L}_j$, $Y_{i}=?$ and none} \\\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \text{of $Y_{i-d+1}^{i}$ is a 1}.\\
	%\mathcal{L}_0,\ \text{if $L_i = \hat{\mathcal{L}}$ and none of $Y_{i-d}^{i}$ is a 1.} 
\end{cases}
\]

The transitions between the labellings can be represented by the finite state machine (FSM) shown in Figure \ref{fig:QUB}. The labellings in conjunction with the message are used to determine the bit $X_{i+1}$ to be transmitted. Formally, $X_{i+1} = \Gamma(m,L_{i+1})$, where the function $\Gamma$ is defined as:

\[\Gamma(m,L_{i+1}) =
\begin{cases}
	0,\ \text{if $L_{i+1} = \mathcal{L}_j$, for some $j$, and}\\ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{$\frac{m-1}{2^{nR}} \notin [\sum_{z<j}\delta_z,\sum_{z\leq j}\delta_z)$},\\
	0,\ \text{if $L_{i+1} = \hat{\mathcal{L}}$},\\
	1,\ \text{if $L_{i+1} = \mathcal{L}_j$, for some $j$, and}\\ \ \ \ \ \ \ \ \ \ \ \ \ \ \text{$\frac{m-1}{2^{nR}} \in [\sum_{z<j}\delta_z,\sum_{z\leq j}\delta_z)$}.
\end{cases}
\]
The chronological order of a single use of the channel at time $i$, for a fixed message $m$, thus is $L_i\rightarrow X_i\rightarrow Y_i$, with $L_{i+1} = G(L_i,Y_{i-d+1}^{i})$.

For a given output sequence $y^i$, we denote by $\mathcal{M}_i$ the set of \emph{possible messages} after time $i$, i.e., $\mathcal{M}_i := \{m\in [2^{nR}]: P(m|y^{i})>0\}$, with $\mathcal{M}_0:=[2^{nR}]$. Note that both the encoder and the decoder can compute the conditional distribution $P(m|y^{i})$ using Bayes' rule. We use the notation $\mathcal{M}_i^{(0)}$ and $\mathcal{M}_i^{(1)}$ to denote the set of messages labelled by a `$0$' and by a `$1$', respectively, in $\mathcal{M}_i$.

A transmission at time $i$ is said to be \emph{successful} if $|\mathcal{M}_i|<|\mathcal{M}_{i-1}|$. Specifically, a successful transmission can occur in one of two scenarios: the first is $y_i = 1$, and the second is where $y_i = 0$ and none of $y_{i-d}^{i-1}$ is a $1$. After a successful transmission, the set of possible messages is calculated and expanded uniformly to the unit interval. It is easy to see that in the first kind of successful transmission, the new set of possible messages, $\mathcal{M}_i$, is equal to $\mathcal{M}_{i-1}^{(1)}$, and in the second kind, $\mathcal{M}_i$ equals $\mathcal{M}_{i-1}^{(0)}$. Figure \ref{fig:succ} shows an illustration of the second of the two kinds of successful transmissions. Figure \ref{fig:eras} depicts the situation when a sequence of erasures is received. In this case, the new set of possible messages, $\mathcal{M}_i$, is equal to $\mathcal{M}_{i-1}$. This transmission procedure continues repeatedly until the set of possible messages contains one message. Additionally, we note that the coding scheme is zero-error, since at the end of the algorithm, the decoder can uniquely decode the transmitted message. The encoding and decoding procedures are described in Algorithm \ref{alg}. 
\begin{figure*}[!t]
	\centering
	
	\includegraphics[width=0.7\textwidth]{Q_graph}
	\caption{Figure shows the finite-state machine (FSM) that represents transitions between the labellings, with the edges labelled by outputs. Note that the state of the FSM can be computed at the encoder using the knowledge of the past $d$ outputs alone. When the encoder is in state $Q_i$, for $i\in \{0,1,\ldots,d\}$, the labelling used is $\mathcal{L}_i$, and when the encoder is in state $\hat{Q}_i$, for $i\in \{0,1,\ldots,d\}$, the labelling used is $\hat{\mathcal{L}}$.}
	\label{fig:QUB}
\end{figure*}

The construction of the labellings ensures that the $(d,\infty)$-RLL input constraint is obeyed. This can be seen from the fact that if ever $Y_i = 1$ for some $i$, it holds that the next $d$ inputs are all set to be $0$s. Further, the staggered manner in which the sub-intervals are labelled by a $1$ in the labellings $\mathcal{L}_0,\ldots,\mathcal{L}_d$ ensures that the input constraint is satisfied when a sequence of erasures is received, too. 

The analysis of the rate of the feedback coding scheme is similar to the proofs of Lemma 3 and Lemma 4 in \cite{0k}. In order to make the exposition self-contained, we repeat parts of the proofs here. For a time index $i\in [n]$, we define $\mathsf{J}_i$ to be the number of information bits gained in a single channel use, which is the logarithm of the change in the size of possible messages at the end of the channel use, i.e.,
\begin{equation}
\label{eq:Jk}
\mathsf{J}_i:= \log_2|\mathcal{M}_{i-1}|-\log_2|\mathcal{M}_{i}|.
\end{equation}
 and $\mathsf{L}_i$ to denote the random variable corresponding to the labelling used, with $\mathsf{L}_i\in \mathcal{L} := \{\hat{\mathcal{L}},\mathcal{L}_0,\ldots,\mathcal{L}_d\}$. The following lemma then holds true:

\begin{lemma}
	\label{lem:gain}
	For any time $i\in [n]$, and for all $\ell\in \mathcal{L}$, we have that $\mathbb{E}[\mathsf{J}_i| \mathsf{L}_i=\ell] = \bar{\epsilon}h_b(\delta_\ell)$, where
	\[\delta_\ell = 
	\begin{cases}
		0,\ \text{if $\ell = \hat{\mathcal{L}}$},\\
		\delta_j,\ \text{if $\ell = \mathcal{L}_j$}.
	\end{cases}
	\]
\end{lemma}
\begin{figure}[!t]
	\centering
	
	\includegraphics[width=0.8\textwidth]{Succ1_2}\label{<figure2>}
	\caption{Figure shows an illustration of a successful transmission of the second kind, when $X_1 = Y_1 = 1$, and when the encoder then transmits $d$ additional zeros. Note that the size of the set of possible messages reduces.}
	\label{fig:succ}
\end{figure}

\begin{figure}[!t]
	\centering
%	\subfloat[]{\includegraphics[width=0.5\linewidth]{Succ1_2}\label{fig:succ}}
%	\hfill
%	\subfloat[]{\includegraphics[width=0.5\linewidth]{Eras_4}\label{fig:eras}}
	\includegraphics[width=0.7\textwidth]{Eras_4}
	\caption{The figure shows the setting when two consecutive erasures are received ($Y_1=Y_2=?$), followed by the successful reception of $X_3 = 1$. So long as erasures are received, the set of possible messages is retained as such, while the labellings cycle through $\mathcal{L}_0$ to $\mathcal{L}_d$. Upon the successful reception of $X_3$, the labelling is changed to $\mathcal{L}_0$. However, since the set of possible messages is now a singleton, the transmission ends with the decoder declaring the correct identity of the message.}
	\label{fig:eras}
\end{figure}

\begin{proof}
	We let the random variable $\theta$ denote the indicator that the current output is unerased, i.e.,
	\[
	\theta_i = \mathds{1}\{Y_i\neq `?'\}.
	\]
	Then,
	\begin{align}
		\mathbb{E}[\mathsf{J}_i|\mathsf{L}_i=\ell]&=\epsilon\mathbb{E}[\mathsf{J}_i|\mathsf{L}_i=\ell,\theta_i = 0]+\bar{\epsilon}\mathbb{E}[\mathsf{J}_i|\mathsf{L}_i=\ell,\theta_i = 1] \notag\\
		&= \bar{\epsilon}\mathbb{E}[\mathsf{J}_i|\mathsf{L}_i=\ell,\theta_i = 1] \label{eq:lemm},
	\end{align}
where the second equality holds since if an erasure is received, the set of possible messages remains the same.

We now note that in any of the labellings $\mathcal{L}_j$, it holds that the length of the sub-interval labelled by a `$1$' equals $\delta_j$, and equals $0$ in $\hat{\mathcal{L}}$. Hence, if labelling $\ell \in \mathcal{L}$ is employed, the bit transmitted is distributed according to Ber$(\delta_\ell)$ \footnote{We note as in \cite{0k} that since the messages are discrete points in $[0,1)$, the transmitted bit is actually distributed according to Ber$(\delta_\ell -e_i)$, where $e_i$ is a correction factor that is bounded as $0\leq e_i\leq \frac{1}{|\mathcal{M}_{i-1}|}$. We use Algorithm \ref{alg} for encoding, until a time $t$ such that $|\mathcal{M}_t|\leq 2^{\lambda}$, for an absolute constant, $\lambda>0$. A clean-up coding phase can then be employed, after the labelling-based scheme, similar to \cite[Appendix C]{SabBEC}, using which the remaining at most $\lambda$ bits are then transmitted. The rate of the overall two-stage coding scheme can then be computed to equal the rate calculated using the analysis in this paper.}, where $\delta_\ell$ is as defined in the statement of the theorem.

 Assume that the current size of the set of possible messages, $\mathcal{M}$, equals $k$, with the current labelling used being $\ell$. If the current bit transmitted is received successfully, then, the new set of possible messages has size $k\delta_\ell$, if the current input bit is a `$1$', and is equal to $k\bar{\delta}_\ell$, otherwise. Hence, the expected number of bits required to describe the new set of possible messages is $\bar{\delta}_{\ell} k \log_2(\bar{\delta}_{\ell} k)+\delta_\ell k \log_2(\delta_\ell k) = \log_2(k)-h_b(\delta_{\ell})$. Thus, given that $\mathsf{L}=\ell$, following a successful transmission, the decoder gains $h_b(\delta_{\ell})$ bits of information. Substituting into \eqref{eq:lemm}, we get that
\[
\mathbb{E}[\mathsf{J}|\mathsf{L}=\ell] = \bar{\epsilon}h_b(\delta_\ell).
\]
\end{proof}

The following lemma computes the rate of the proposed coding scheme:
\begin{lemma}
	\label{lem:rate}
	For any $\epsilon \in [0,1]$, the proposed coding scheme achieves a rate
	\[
	R = \max_{\vec{\delta}\in \Delta_d} R(\vec{\delta}),
	\]
	where $R(\vec{\delta})$ is as defined in equation \eqref{eq:R}.
\end{lemma}
\begin{proof}
	Fix $0\leq \delta_0,\delta_1,\ldots,\delta_d\leq 1$, with $\sum_{i=0}^{d}\delta_i \leq 1$. The constraint is chosen so as to ensure that the lengths of the intervals used in the labellings in Figure \ref{fig:labellings} are all non-negative. 
	
	Consider the Markov chain induced by the transitions shown in Figure \ref{fig:QUB}, with the transition probabilities $P(Y=?|q) = \epsilon$, for all $q \in \{Q_0,Q_1,\ldots,Q_d,\hat{Q}_0,\hat{Q}_1,\ldots,\hat{Q}_d\}$, and
	\[
	P(Y=1|q) = 
	\begin{cases}
		\bar{\epsilon}\delta_i, \ \text{if $q = Q_i$, for some $i$},\\
		0, \ \text{otherwise}.
	\end{cases}
	\]
	Let $\pi(\ell)$ denote the stationary probability of using labelling $\ell$, which can be calculated using the stationary probabilities of states of the Markov chain on the FSM. Clearly, for $i\in \{0,1,\ldots,d\}$, $\pi(\mathcal{L}_i)$ equals $\pi(Q_i)$, and $\pi(\hat{\mathcal{L}})$ equals $\sum_{j=0}^{d}\pi(\hat{Q}_j)$. The rate of the coding scheme can be computed to be:
	\begin{align*}
		R &= \lim_{n\rightarrow \infty}  \frac{\log_2 |\mathcal{M}_0|}{n}\\
		&\stackrel{(a)}{=} \lim_{n\rightarrow \infty} \frac{1}{n}\sum_{k=1}^{n}\mathbb{E}[\mathsf{J}_k]\\
		&= \lim_{n\rightarrow \infty}  \frac{1}{n} \sum_{k=1}^{n} \sum_{\ell \in \mathcal{L}} P(\mathsf{L}_k = \ell)\mathbb{E}[\mathsf{J}_k|\mathsf{L}_k = \ell]\\
		&\stackrel{(b)}{=} \sum_{\ell \in \mathcal{L}} \bar{\epsilon}h_b(\delta_\ell) \lim_{n\rightarrow \infty}  \frac{1}{n} \sum_{k=1}^{n} P(\mathsf{L}_k = \ell)\\
		&\stackrel{(c)}{=} \sum_{\ell \in \mathcal{L}} \bar{\epsilon}h_b(\delta_\ell)\pi(\ell)\\
		&= \sum_{i=0}^{d}\bar{\epsilon}h_b(\delta_i)\pi(\mathcal{L}_i)\\
		&\stackrel{(d)}{=} R(\vec{\delta}),
	\end{align*}
where 
\begin{enumerate}[label = (\alph*)]
	\item holds from equation \eqref{eq:Jk},
	\item follows from Lemma \ref{lem:gain} and by exchanging the order of the summations,
	\item follows from the definition of stationary probability and from the fact that the random process $(\mathsf{L}_n:n\in \mathbb{N})$ is a positive recurrent, irreducible, aperiodic Markov chain (this follows from the irreducibility and aperiodicity of the graph in Figure \ref{fig:QUB}), and
	\item holds by an explicit calculation of the stationary probabilities of the Markov process $(\mathsf{L}_n:n\in \mathbb{N})$, which are given by:
	\[
	\pi(\ell)=
	\begin{cases}
		\frac{\epsilon^i}{\sum_{j=0}^{d}\epsilon^j + d\bar{\epsilon}\left(\sum_{j=0}^{d}\epsilon^j\delta_j\right)},\ \ell=\mathcal{L}_i,\\
		\frac{d\bar{\epsilon}\left(\sum_{j=0}^{d}\epsilon^j\delta_j\right)}{\sum_{j=0}^{d}\epsilon^j + d\bar{\epsilon}\left(\sum_{j=0}^{d}\epsilon^j\delta_j\right)},\ \ell=\hat{\mathcal{L}}.
	\end{cases}
	\]
\end{enumerate}
Therefore, maximizing over all allowed parameters $\delta_0,\ldots,\delta_d$, it follows that our coding scheme achieves a rate $R = \max_{\vec{\delta}\in \Delta_d} R(\vec{\delta})$.
\end{proof}

We now provide an upper bound on the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC, using Theorem \ref{thm:UB}.
\begin{lemma}
	\label{lem:ub}
	For any $\epsilon \in [0,1]$, the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC is bounded as:
	\[
	C^{\text{fb}}_{(d,\infty)}\leq \max_{\vec{\delta}\in \Delta_d} R(\vec{\delta}).
	\]
\end{lemma}
\begin{proof}
	We simply apply Theorem \ref{thm:UB} to the $Q$-graph that is the FSM in Figure \ref{fig:QUB}. The transition probabilities $P(Y=y|q)$ are the same as those in the proof of Lemma \ref{lem:rate}, for $y\in \{0,?,1\}$ and $q \in \{Q_0,Q_1,\ldots,Q_d,\hat{Q}_0,\hat{Q}_1,\ldots,\hat{Q}_d\}$. Note that the definition of the transition probabilities implies that 
	\[
	P(X=1|q) = 
	\begin{cases}
		\delta_i, \ \text{if $q = Q_i$, for some $i$},\\
		0, \ \text{otherwise}.
	\end{cases}
	\]
	 We then have that
	 \begin{align*}
	 	I(X;Y|Q) &\stackrel{(a)}{=} H(Y|Q) - H(Y|X)\\
	 	&= H(Y|Q) - h_b(\epsilon)\\
	 	&\stackrel{(b)}{=} \bar{\epsilon}H(X|Q)+h_b(\epsilon) - h_b(\epsilon)\\
	 	&= \sum_{\ell \in \mathcal{L}} \bar{\epsilon}h_b(\delta_\ell)\pi(\ell)\\
	 	&= \sum_{i=0}^{d}\bar{\epsilon}h_b(\delta_i)\pi(\mathcal{L}_i)\\
	 	&= R(\vec{\delta}),
	 \end{align*}
 where
 \begin{enumerate}[label = (\alph*)]
 	\item holds due to the memorylessness of the BEC, and
 	\item follows from the simple identity that $H(a\bar{c},\bar{a}\bar{c},c) = h_b(c)+\bar{c}h_b(a)$, for all $a,c \in [0,1]$.
 \end{enumerate}
Hence, all that remains to be shown for the proof to be complete is that 
\[
\sup_{\{P(x|s,q)\}} R(\vec{\delta}) = \max_{\sum_{i=0}^{d}\delta_i \leq 1}R(\vec{\delta}).
\]
This is true since for any valid input distribution $\{P(x|s,q)\}$ on the $(S,Q)$-graph corresponding to the $Q$-graph in Figure \ref{fig:QUB}, it holds that
\begin{align*}
	\sum_{i=0}^{d}\delta_i = \sum_{i=0}^{d}P(X=1|Q_i)
	&= \sum_{i=0}^{d}\frac{P(X=1,Q_i)}{\pi(\mathcal{L}_i)}\\
	&{=} \sum_{i=0}^{d}\frac{P(X=1,Q_i)}{\epsilon^i \pi(\mathcal{L}_0)}\\
	&= \frac{1}{ \pi(\mathcal{L}_d)}\sum_{i=0}^{d}\epsilon^{d-i}P(X=1,Q_i).	
\end{align*}
Now,
\begin{align*}
    \sum_{i=0}^{d}\delta_i &= \frac{1}{ \pi(\mathcal{L}_d)}\sum_{i=0}^{d}\epsilon^{d-i}P(X=1,Q_i)\\
    &= \frac{1}{ \pi(\mathcal{L}_d)}\sum_{i=0}^{d}\epsilon^{d-i}P(X=1,S=d,Q_i)\\
    &\leq \frac{1}{ \pi(\mathcal{L}_d)}\left(\sum_{i=0}^{d-1}\epsilon^{d-i}P(X=1,S=d,Q_i)+P(S=d,Q_d)\right)\\
    &= \frac{1}{ \pi(\mathcal{L}_d)}\left(\sum_{i=0}^{d-1}P(S=i,Q_d)+P(S=d,Q_d)\right)\\
    &=1,
\end{align*}
where the penultimate equality holds from the structure of the $(S,Q)$-graph.
\end{proof}
\begin{remark}
	We note that for the case when $d=2$, the authors in \cite{0k} provide the optimal $Q$-graph of Figure \ref{fig:QUB} for evaluating an upper bound on the feedback capacity. We have shown here that their upper bound is tight.
\end{remark}
Lemmas \ref{lem:rate} and \ref{lem:ub}, taken together, prove Theorem \ref{thm:main}. We thus obtain an exact characterization of the feedback capacity, in addition to providing an explicit coding scheme.

==> introduction.tex <==

Discrete memoryless channels (DMCs) were introduced by Shannon \cite{Sh48} as models for communication links, and have, since then, been the object of much research activity in information theory. It was shown by Shannon \cite{Sh56} that causal, noiseless feedback of the outputs does not increase the capacity of memoryless channels, which is given by $C = \sup_{P(x)}I(X;Y)$.


In this paper, we consider DMCs with input constraints, which are specific instances of discrete channels with memory, and which find application in magnetic and optical recording systems \cite{Roth}, \cite{Immink}. Such channels fall under the broad category of finite-state channels (or FSCs), the numerical computation of whose non-feedback capacities has been considered in works such as \cite{GBAA} and \cite{Han3}. Figure \ref{fig:genconstdmc} shows a generic DMC with input constraints, with causal, noiseless feedback. The computation of the feedback capacity of an FSC using a dynamic programming (DP) formulation first appeared in \cite{Chen} and was later extended in works such as \cite{Tatikonda1} and \cite{Tatikonda2}. In this work, we shall focus on the binary erasure channel (or BEC), the inputs of which are constrained to obey the $(d,\infty)$-runlength limited (RLL) input constraint\footnote{The $(d,\infty)$-RLL constraint is a special case of the $(d,k)$-RLL constraint on binary sequences, which requires that the length of any run of consecutive $0$s is at least $d$ and at most $k$.}, which mandates that there needs to be at least $d$ $0$s between any pair of successive $1$s. Such RLL input constraints are necessary for mitigating inter-symbol interference and timing and synchronization errors. As was shown in the works \cite{SabBEC}, \cite{Hanerasure}, and \cite{SabBIBO}, the capacities of the $(1,\infty)$-RLL input-constrained binary erasure and binary symmetric channels are strictly larger than their respective non-feedback capacities, for at least some values of the channel parameters, thereby demonstrating that for channels with memory, feedback may indeed increase capacity.

\begin{figure}[!t]
	\centering
	\includegraphics[scale=0.4]{genconstdmc.png}
	\caption{System model of an input-constrained DMC with causal, noiseless feedback.}
	\label{fig:genconstdmc}
\end{figure}

In the context of the BEC with input constraints, the feedback capacities of the $(1,\infty)$- and the $(0,k)$-RLL input constraints (for $k\geq 1$) were computed in the works \cite{SabBEC} and \cite{0k}, respectively. Both of these works put down an explicit coding scheme, whose rate equals the capacity of the BEC with non-causal knowledge of erasures\footnote{Informally, the non-causal capacity is the maximum achievable rate of a coding scheme for the BEC in a setting in which the encoder knows, \emph{prior} to the transmission of the $i^{\text{th}}$ bit $x_i$, whether or not $x_i$ will be erased.}, which, in turn, is as an upper bound on the feedback capacity. Interestingly, this gives rise to the fact that the non-causal capacities of the BEC with the $(1,\infty)$- and the $(0,k)$-RLL input constraints are equal to the respective feedback capacities. Moreover, it was shown in \cite{0k} that the feedback capacity of the $(2,\infty)$-RLL input-constrained BEC is less than the corresponding non-causal capacity, when the channel parameter, $\epsilon$, is equal to $0.5$. In this paper, we show that for the $(2,\infty)$-RLL input-constrained BEC, the feedback capacity is in fact equal to the non-causal capacity for $\epsilon\in [0,1-\frac{1}{2\log(3/2)}]$. This result is a by-product of the main theorem in our paper, which presents an analytical lower bound on the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC, for all $d$ greater than or equal to $1$. For the case when $d=1$, our lower bound is tight for all values of $\epsilon$ \cite{SabBEC}, and for $d=2$, our lower bound is numerically close to an upper bound derived using techniques in \cite{Graph_based}, for $\epsilon$ larger than $1-\frac{1}{2\log(3/2)}$, too. We also present analytical upper bounds on the feedback capacity of the $(d,\infty)$-RLL input-constrained BEC, which, like our lower bounds, are single-parameter optimization problems. We observe that our bounds differ from the non-causal capacity expression (see \cite{0k}) in only the domain of maximization. 

Our techniques involve the use of the single-letter bounding techniques of Sabag et al. in \cite{Single}, and we come up with a specific $Q$-graph (or a $Q$-context mapping) and a choice of a specific ``BCJR-invariant'' input distribution, which gives rise to an achievable rate.

==> preamble.tex <==
% preamble.tex

\geometry{letterpaper, top=2.2in, headheight=1.7in}
\date{}

\makeatletter

\def\fulltitle#1{\def\@fulltitle{#1}}
\def\runningtitle#1{\def\@runningtitle{#1}}
\def\runningauthor#1{\def\@runningauthor{#1}}
\def\affiliation#1{\def\@affiliation{#1}}
\def\department#1{\def\@department{#1}}
\def\memoid#1{\def\@memoid{#1}}
\def\theyear#1{\def\@theyear{#1}}
\def\mydate#1{\def\@mydate{#1}}

\runningtitle{How to write an effective report} % Short title
\author{Your name \and John Doe \and Jane Doe} % Full list of authors
\runningauthor{Your name et al.} % Short list of authors
\affiliation{Your University} % Affiliation e.g. University or Company
\department{Your Department} % Department or Office
\memoid{AI Memo 777} % ID of the tech report
\theyear{2018} % year of the tech report
\mydate{August 08, 2018} %the date

\def\displaymydate{\@mydate}
\def\displaytheyear{\@theyear}
\def\displaymemoid{\@memoid}
\def\displaydepartment{\@department}
\def\displayaffiliation{\@affiliation}
\def\displayrunningauthor{\@runningauthor}
\def\displayrunningtitle{\@runningtitle}

\makeatother

\makeatletter
\patchcmd{\@zfancyhead}{\fancy@reset}{\f@nch@reset}{}{}
\patchcmd{\@set@em@up}{\f@ncyolh}{\f@nch@olh}{}{}
\patchcmd{\@set@em@up}{\f@ncyolh}{\f@nch@olh}{}{}
\patchcmd{\@set@em@up}{\f@ncyorh}{\f@nch@orh}{}{}
\makeatother

% ----------
% fancyhdr setup
% ----------

\pagestyle{fancy}
\renewcommand{\headrulewidth}{0pt}

\fancypagestyle{firstpage}
{
    \fancyhf{}
    \fancyhead{%
        \begin{center}
            \textsc{\displayaffiliation}\\
            \textsc{\displaydepartment}
        \end{center}
        \vspace*{0.5in}
        \displaymemoid
        \hfill
        \displaymydate
    }
    \fancyfoot[L]{\footnotesize \textbf{\textsc{\displayaffiliation} -- \displaytheyear}}
}
\fancyhead[EL]{\small \displayrunningauthor}
\fancyhead[ER]{\small Page \thepage}
\fancyhead[OL]{\small Page \thepage}
\fancyhead[OR]{\small \displayrunningtitle}

\chead{}
\lfoot{}
\cfoot{}
\rfoot{}

% ----------

\providecommand{\keywords}[1]{\noindent \textbf{Keywords:} #1} % keywords definition

\renewcommand{\familydefault}{\sfdefault} % sans-serif font
\setlength{\parskip}{1em} % 1em skip between paragraphs
\abslabeldelim{:} % use colon after the run-in 'Abstract' word
\setlength{\parindent}{0pt} % no indentantion for first page 
\setlength{\abstitleskip}{-\absparindent} % this is because the abstract package sets \absparindent to \parindent

\pretitle{\Large \begin{center}}
\posttitle{\\[2ex] \Large \textbf{by}\end{center}}

==> report_header.tex <==
\usepackage{ifthen}
\usepackage{cite}
\usepackage{algorithm}
\usepackage[cmex10]{amsmath} % Use the [cmex10] option to ensure complicance
% with IEEE Xplore (see bare_conf.tex)
\usepackage{amsthm,amsfonts,amssymb}
\usepackage[noend]{algpseudocode}
\setcounter{MaxMatrixCols}{17}

\usepackage{subfig}
\usepackage{blkarray}
\usepackage[mathscr]{euscript}
\usepackage{enumitem}
%\usepackage{romannum}
\usepackage{blkarray}
\usepackage{stfloats}%
%\newtheorem{theorem}{Theorem}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{lemma}[section]{Lemma}
\theoremstyle{remark}
\newtheorem*{remark}{Remark}
\theoremstyle{definition}
\newtheorem{definition}{Definition}[section]
%\theoremstyle{definition}
%\newthorem{definition}{Definition}[section]
%\usetikzlibrary{graphs}
\usepackage{url}
\usepackage{arydshln}
\usepackage{mathtools}
\usepackage{dsfont}
%\usepackage{kbordermatrix}
%\newcommand{\indicator}[1]{\mathbb{1}_{\set{#1}}}
%\usepackage{braket}
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor} % Use the [cmex10] option to ensure complicance
% with IEEE Xplore (see bare_conf.tex)

\usepackage{geometry}
\usepackage[utf8]{inputenc}
\usepackage[english]{babel}
\usepackage[runin]{abstract}
\usepackage{titling}
\usepackage{booktabs}
\usepackage{fancyhdr}
\usepackage{helvet}
\usepackage{csquotes}
\usepackage{graphicx}
\usepackage{blindtext}
\usepackage{parskip}
\usepackage{etoolbox}


==> rm.tex <==
\label{sec:rm}
%(\textbf{Delete from here})
%In this section, we consider the BMS channel with the $(d,\infty)$-RLL input constraint, but in the absence of feedback. We first recall some well-known results on the capacity without feedback of general input-constrained discrete memoryless channels (DMCs).
%\begin{theorem}[\cite{Gallager}, Chap. 4, \textsection 6]
%	The capacity of an input-constrained DMC without feedback is given by:
%	\[
%	C_{\text{ic-DMC}} = \lim_{N\rightarrow \infty} \max_{P(x^N)}\frac{1}{N} I(X^N;Y^N),
%	\]
%	where the maximum is taken over input distributions, $\{P(x^N)\}$, which satisfy the input constraint.
%\end{theorem}
%The expression above is a multi-letter mutual information expression, the explicit computation of which is a well-known open problem. A common technique for lower bounding the capacity is the restriction of the input process to be a stationary and ergodic Markov process of finite order. This procedure is meaningful in the context of results such as those in \cite{chen} and \cite{litan}, which show that the capacity of any indecomposable FSC (of which input-constrained DMCs form a special class) can be approached arbitrarily closely by a sequence of stationary and ergodic Markov processes of increasing order. However, such results do not reveal insight into the capacity expression.
%
%For the case when the input process is first-order Markov, some analytical lower bounds are known (see, for example, \cite{ZW88, Han2, arnk20, arnk21ncc}). We put down here the simplest of these results, which pertains to the input-constrained BEC with a $(d,k)$- or $(d,\infty)$-RLL input constraint.
%\begin{lemma}[\cite{arnk20}, Theorems V.3 and V.4]
%	\label{lem:linearlb}
%	The capacity of the BEC with a $(d,k)$- or $(d,\infty)$-RLL input constraint is lower bounded as:
%	\[
%	C_{(d,k)}(\epsilon) \geq C_0^{(d,k)}\cdot (1-\epsilon);\quad C_{(d,\infty)}(\epsilon) \geq C_0^{(d,\infty)}\cdot (1-\epsilon).
%	\]
%\end{lemma}
%However, the bounds above do not specify low-complexity encoding and decoding schemes that achieve the rates mentioned. Our objective is to identify explicit families of fixed-length codes that involve low complexity encoding and decoding procedures, and which achieve non-trivial rates over the $(d,\infty)$-RLL input-constrained BEC. 
%
%(\textbf{Upto here})

As mentioned in Section \ref{sec:main}, we consider the Reed-Muller (RM) family of codes, $\{\mathcal{C}_m(R)\}$, which are such that any rate $R\in [0,C)$ is $(0,\infty)$-achievable (see Definition \ref{def:ach}) over the BMS channel (see Theorem \ref{thm:Reeves}), where $C$ denotes the capacity of the channel. We then select linear subcodes that respect the $(d,\infty)$-RLL constraint, of such a capacity-achieving sequence of RM codes, and compute their rate. For notational convenience, we denote by $S_{(d,\infty)}^{(n)}$, the set of $n$-length binary vectors that respect the $(d,\infty)$-RLL constraint, i.e.,
\begin{align*}
S_{(d,\infty)}^{(n)}:=\bigl\{\mathbf{c} = (c_0,\ldots,c_{n-1}): \mathbf{c}&\text{ respects the $(d,\infty)$-RLL}\\ &\text{ input constraint}\bigr\}.
\end{align*}
%Likewise,
%\begin{align*}
%	S_{(0,k)}^{(n)}:=\bigl\{\mathbf{c} = (c_0,\ldots,c_{n-1}): \mathbf{c}&\text{ respects the $(0,k)$-RLL}\\ &\text{ input constraint.}\bigr\}.
%\end{align*}
We suppress the superscript `$(n)$' if the length of the vector is clear from the context.

We begin with a simple observation, presented below as a lemma. We recall that the support of a vector $\mathbf{c}\in \mathbb{F}_2^{n}$,
\[
\text{supp}(\mathbf{c}) = \{i: c_i = 1\}.
\]

\begin{lemma}
	\label{lem:simplerm}
	Given $d\geq 1$, if $\hat{\mathbf{c}}$ is such that $\hat{\mathbf{c}}\in S_{(d,\infty)}$, and supp$(\mathbf{c}) \subseteq \text{supp}(\hat{\mathbf{c}})$, then it holds that $\mathbf{c}\in S_{(d,\infty)}$.
\end{lemma}
%\begin{proof}
%	The proof is simply that if $\hat{\mathbf{c}}$ respects the $(d,\infty)$-RLL constraint, there are at least $d$ $0$s between successive $1$s, and since supp$(\mathbf{c}) \subseteq \text{supp}(\hat{\mathbf{c}})$, it is true that the same property holds for $\mathbf{c}$ as well.
%\end{proof}
%The proof follows from the definition of the support of a binary vector, and is omitted here.

%The proof of Theorem \ref{thm:rm} is given below. We use the convenient notation ${n\choose \leq k}$ to denote $\sum_{i=0}^{k}{n\choose i}$.

Another fact that we repeatedly use is recorded in Lemma~\ref{lem:rate} below. For this, recall our definition of $r_m$ from \eqref{eq:rmval}.
% is such that the rate of the code $\text{RM}(m,r_m)$ converges to $R$ as $m \to \infty$, i.e., $\lim\limits_{m \to \infty} \frac{1}{2^m} \, \binom{m}{\le r_m} = R$. 

\begin{lemma}
\label{lem:rate}
For any sequence of positive integers $(t_m)$ such that $t_m = o(\!\!\sqrt{m})$, we have
$$
\lim_{m \to \infty} \frac{1}{2^{m-t_m}} \binom{m-t_m}{\le r_m} \ = \ R.
$$
In particular, for any fixed integer $t > 0$, $\lim\limits_{m \to \infty} \frac{1}{2^m} \binom{m-t}{\le r_m} = 2^{-t}R$.
\end{lemma}
\begin{proof}
Let $S_m$ denote a Bin$(m,\frac12)$ random variable, and note that $\frac{1}{2^{m-t_m}} \binom{m-t_m}{\le r_m}$ equals $\Pr[S_{m-t_m} \le r_m]$. Further note that by our choice of $r_m$, for any integer $t > 0$, we have for all $m$ large enough,
\begin{align}
	|r_m - r_{m-t}| &\leq \biggl| \frac{m}{2} + \frac{\sqrt{m}}{2}Q^{-1}(1-R) \, - \notag\\
	   &\ \ \ \ \ \ \ \ \ \ \ \left(\frac{m-t}{2} + \frac{\sqrt{m-t}}{2}Q^{-1}(1-R)\right) + 1 \biggr| \notag\\
	&\leq \frac{t}{2}+\frac{\sqrt{t}}{2}\lvert Q^{-1}(1-R)\rvert + 1. \label{eq:rm_diff}
\end{align}
Hence, we have $r_{m-t_m} - \nu_m \le r_m \le r_{m-t_m} + \nu_m$, with $\nu_m := \frac{t_m}{2}+\frac{\sqrt{t_m}}{2}\lvert Q^{-1}(1-R)\rvert + 1$.
Consequently, $\Pr[S_{m-t_m} \le r_{m-t_m} - \nu_m] \le \Pr[S_{m-t_m} \le r_m] \le \Pr[S_{m-t_m} \le r_{m-t_m} + \nu_m]$. Setting $\overline{S}_{m-t_m} := \frac{S_{m-t_m} - \frac12(m-t_m)}{\frac12\sqrt{m-t_m}}$, we have 
\begin{align}
& \Pr[\overline{S}_{m-t_m} \le Q^{-1}(1-R) - \frac{\nu_m}{\frac12\sqrt{m-t_m}}] \notag \\
& \ \ \ \ \ \le \ \Pr[S_{m-t_m} \le r_m] \notag \\
& \ \ \ \ \ \ \ \ \ \ \ \le \ \Pr[\overline{S}_{m-t_m} \le Q^{-1}(1-R) + \frac{\nu_m}{\frac12\sqrt{m-t_m}}].
\label{sandwich}
\end{align}

Now, by the central limit theorem (or, in this special case, by the de Moivre-Laplace theorem), $\overline{S}_{m-t_m}$ converges in distribution to a standard normal random variable, $Z$. Therefore, via \eqref{sandwich} and the fact that $t_m$ and $\nu_m$ are both $o(\!\!\sqrt{m})$, we obtain that 
$$
\lim_{m \to \infty} \Pr[S_{m-t_m} \le r_m]  \ = \ \Pr[Z \le Q^{-1}(1-R)] \ = \ R,
$$
which proves the lemma.
\end{proof}

We are now in a position to prove Theorem~\ref{thm:rm}.

\begin{proof}[Proof of Theorem~\ref{thm:rm}]
	For a fixed $d\geq 1$, let $z := \left \lceil \log_2(d+1)\right \rceil$. Consider the subcode $\mathcal{C}_m^{(d,\infty)}(R)$, of the code $\mathcal{C}_m(R)$, defined as:
	\begin{align}
		\label{eq:rmlb1}
	\mathcal{C}_m^{(d,\infty)}(R):=\Bigg\{\text{Eval}(f): f = &\bigg(\prod_{i=m-z+1}^{m} x_i \bigg)\cdot g(x_{1},\ldots, x_{m-z}),\\ &\text{ where } \text{deg}(g)\leq r_m-z\Bigg\}.
	\end{align}
The fact that the code $\mathcal{C}_m^{(d,\infty)}(R)$ is linear, is clear. Further, it can be verified that the polynomial $h(x_{m-z+1},\ldots,x_m):=\prod_{i=m-z+1}^{m} x_i$ is such that its corresponding evaluation vector, Eval$(h)$, obeys Eval$(h)\in S_{(d,\infty)}^{(2^m)}$. This is because Eval$_\mathbf{y}(h) = 1$ if and only if $(y_{m-z+1},\ldots,y_m) = (1,\ldots,1)$, and in the lexicographic ordering, such evaluation points $\mathbf{y}$ are spaced out by $2^z - 1$ coordinates, where $2^z-1\geq d$. Thus, for any polynomial $f$ such that $\text{Eval}(f)\in \mathcal{C}_m^{(d,\infty)}(R)$, it is true that supp$(\text{Eval}(f))\subseteq \text{supp}(\text{Eval}(h))$, so that Eval$(f) \in S_{(d,\infty)}^{(2^m)}$ via Lemma \ref{lem:simplerm}. Hence, for any $R\in (0,1)$, it holds that $\mathcal{C}_m^{(d,\infty)}(R)$ is a collection of RM codewords in $\mathcal{C}_m(R)$, all of which respect the input constraint.

Consequently, the rate of the subcode $\mathcal{C}_m^{(d,\infty)}(R)$ is
\begin{align*}
	R_m^{(d,\infty)} \ & =\ \frac{\log_2(|\mathcal{C}_m^{(d,\infty)}|)}{2^m} \\ 
	&= \ \frac{{m-z \choose \leq r_m-z}}{2^m} 
		\ = \ \frac{\binom{m-z}{\le r_m-z}}{\binom{m-z}{\le r_m}} \, \frac{{m-z \choose \leq r_m}}{2^m}
		\ \xrightarrow{m \to \infty} \ 2^{-z}R.
\end{align*}
 To obtain the limit as $m \to \infty$, we have used Lemma~\ref{lem:rate} and the fact that the ratio $\frac{\binom{m-z}{\le r_m-z}}{\binom{m-z}{\le r_m}}$ converges to $1$ as $m \to \infty$.
\end{proof}
%(\textbf{Delete this Remark})
%\begin{remark}
%	We note, for example, when $d=1$, the rate calculated in Theorem \ref{thm:rm}, when using the sequence of codes $\{\mathcal{C}_m^{(d,\infty)}(1-\epsilon)\}$, is $\frac{1}{2}(1-\epsilon)$, which is less than the lower bound of $\approx 0.694\cdot(1-\epsilon)$, obtained from Lemma \ref{lem:linearlb}. However, we have identified, explicitly, a set of codewords that, when sent over an BEC, can be decoded using low-complexity decoders for RM codes (see, for example, \cite{rm_survey}).
%\end{remark}

%The proof of Theorem \ref{thm:0k} is similar to that of Theorem \ref{thm:rm}, and is stated below.
%\begin{proof}
%    For a fixed $k\geq 1$, let $t:= \left \lfloor \log_2(k+1)\right \rfloor$. Consider the subcode $\mathcal{C}_m^{(0,k)}(R)$, of the code $\mathcal{C}_m(R)$, defined as:
%	\begin{align}
%	\label{eq:0kconst}
%	&\mathcal{C}_m^{(0,k)}(R):=\{\text{Eval}(f): f = 1+(1+x_S)\cdot g(x_{1},\ldots, x_{m-t}),  \notag\\ &\text{ where }S\neq \emptyset, S \subseteq [m-t+1:m], \text{ and }\text{deg}(g)\leq r_m-|S|\}.
%	\end{align}
%	It can be checked that $\mathcal{C}_m^{(0,k)}(R)$ consists of only codewords $\mathbf{c}\in S_{(0,k)}^{(2^m)}$, via Lemma \ref{lem:simplerm}, and using the fact that Eval$(x_S)$ has runs of $0$s of length at most $2^t$, for $S$ as in \eqref{eq:0kconst}. It then holds that Eval$((1+x_S))$ has runs of $1$s of length at most $2^t$, and since supp$(\text{Eval}((1+x_S)g))\subseteq \text{supp}(\text{Eval}(1+x_S))$, the desired property of Eval$(f)$ readily follows. 
%	
%	Again, by simple calculations, it follows that the rate of the subcode
%	\begin{align}
%	R_m^{(0,k)}&=\frac{\log_2(|\mathcal{C}_m^{(0,k)}|)}{2^m} \notag\\
%		&\stackrel{(a)}{\geq} \frac{\log_2\left(2^t\cdot \text{exp}_2\left({m-t \choose \leq r_m-t}\right)\right)}{2^m}\notag\\
%		& = \frac{1}{2^t} \cdot \frac{t+{m-t \choose \leq r_m-t}}{2^{m-t}}\notag\\
%		&\xrightarrow[m \to \infty]{} 2^{-t}R, \notag
%\end{align}
%where (a) follows from the fact that for each of the $2^t$ non-empty subsets $S\subseteq[m-t+1:m]$, there are at least $\text{exp}_2\left({m-t \choose \leq r_m-t}\right)$ polynomials $g(x_1,\ldots,x_{m-t})$, having degree at most $r_m-t$. Further, the limit in the last step follows from the arguments in equation \eqref{eq:rmbound1}.% and \eqref{eq:rmbound2}.
%\end{proof}
\begin{remark}
	The achievable rate calculated in this paper supplements the results of \cite{pvk}, which show the existence of $(d,\infty)$- and $(0,k)$-RLL) subcodes of cosets of any $(0,\infty)$-capacity-achieving linear code, over a BMS channel with capacity $C$, of rate at least $C_0 + C-1$, where $C_0$ is the noiseless capacity of the input constraint. In particular, the paper shows the existence of codes of rate at least $C_0-\epsilon$, for the BEC$(\epsilon)$, and $C_0 - h_b(p)$, for the BSC$(p)$. However, the paper does not provide an explicit identification of such codes. We note in addition that our achievable rate exceeds the lower bounds in \cite{pvk}, for large $\epsilon$, over the BEC, and for $p$ close to $0.5$, over the BSC.
\end{remark}
In the context of the design of coding schemes over (input-constrained) BMS channels, it would be remiss to not comment on the rates achieved by polar codes, given that polar codes are capacity-achieving over a broad class of channels (see, for example, \cite{polar}, \cite{tal}, \cite{tal2}, and reference therein). Following the work of Li and Tan in \cite{litan}, and as pointed out earlier, it holds that the capacity without feedback of the class of input-constrained DMCs can be approached arbitrarily closely using stationary, ergodic Markov input distributions of finite order. Moreover, from \cite{polarmemory}, it can be verified that polar codes do achieve the information rates over a BMS channel, of any stationary, ergodic finite-state Markov input process
%, that satisfy a certain ``forgetfulness'' property, a sufficient condition for which is given by Condition K in the paper. 
In particular, this shows that polar codes do achieve the capacity of  $(d,\infty)$- and $(0,k)$-RLL input-constrained BMS channels. However, this observation is not very helpful for the following reasons:
\begin{itemize}
	\item We do not possess knowledge of an optimal sequence of Markovian input distributions.
	\item Polar codes are (structured) random codes, and the exact choice of the bit-channels to send information bits over, requires analysis. In our construction, however, we have explicitly identified the codewords being transmitted.
	\item Finally, this observation does not lend insight into explicit lower bounds on non-feedback capacity.
\end{itemize}

==> rmub.tex <==
\label{sec:rmub}
In this section, we provide upper bounds on the rates over a $(1,\infty)$-RLL input-constrained BMS channel, achievable using subcodes (not necessarily linear) of $\{\mathcal{C}_m(R)\}$ (see \eqref{eq:rmval}), which is a $(0,\infty)$-capacity-achieving family of RM codes. We fix the co-ordinate ordering to be the standard lexicographic ordering. %For simplicity, we first present the analysis for the case when $d=1$, and extend the arguments to general $d$, later.

Following the expositions in \cite[Chap. 13]{mws} and \cite{rm_survey}, it holds that any Boolean polynomial $f \in \mathbb{F}_2[x_1,\ldots,x_m]$, such that Eval$(f) \in \text{RM}(m,r)$, can be expressed as:
\begin{equation}
	\label{eq:rmdecomp}
f(x_1,\ldots,x_m) = g(x_1,\ldots,x_{m-1}) + x_m\cdot h(x_1,\ldots,x_{m-1}), 
\end{equation}
where $g,h$ are such that Eval$(g)\in \text{RM}(m-1,r)$ and Eval$(h)\in \text{RM}(m-1,r-1)$. The following lemma then holds true:
\begin{lemma}
	\label{lem:necesscond}
	If a codeword Eval$(f)\in \text{RM}(m,r)$ is such that Eval$(f)\in S_{(1,\infty)}$, then, supp$(\text{Eval}(g)) \subseteq \text{supp}(\text{Eval}(h))$, where $g,h$ are as in \eqref{eq:rmdecomp}.
\end{lemma}
\begin{proof}
	Suppose that there exists some evaluation point $\mathbf{z} = (z_1,\ldots,z_{m-1}) \in \mathbb{F}_2^{m-1}$ such that $g(\mathbf{z})=1$ and $h(\mathbf{z})=0$. Then it follows that at evaluation points $\mathbf{z}_1,\mathbf{z}_2 \in \mathbb{F}_2^m$ such that $\mathbf{z}_1 = \mathbf{z}0$ and $\mathbf{z}_1 = \mathbf{z}1$, it holds that $f(\mathbf{z}_1) = f(\mathbf{z}_2) = 1$. Since by construction the points $\mathbf{z}_1$ and $\mathbf{z}_2$ are consecutive in the lexicographic ordering, the codeword Eval$(f)\notin S_{(1,\infty)}$. 
\end{proof}
%\begin{remark}
%	In fact, a simple, sufficient condition can also be derived for Eval$(f)\in \text{RM}(m,r)$ to respect the $(1,\infty)$-RLL constraint, by requiring that $h$ take on the value of $1$ at points just prior to the start of a run of $1$s in Eval$(g)$. However, since this condition is not required for the upper bounding technique, we omit a detailed description. 
%\end{remark}
Now consider any sequence of RM codes, $\{{\mathcal{C}}_m(R)\}$, where ${\mathcal{C}}_m(R) = \text{RM}(m,r_m)$, where $r_m$ is as in \eqref{eq:rmval}. By Theorem \ref{thm:Reeves}, we know that the sequence $\{\mathcal{C}_m(R)\}$ achieves a rate of $R\in (0,C)$, where $C$ is the capacity of the unconstrained BMS channel. From Lemma \ref{lem:necesscond}, it follows that in order to obtain an upper bound on the number of codewords, Eval$(f) \in {\mathcal{C}}_m(R)$, that respect the $(1,\infty)$-RLL constraint, it is sufficient to obtain an upper bound on the number of polynomials $h$, for a given $g$, such that supp$(\text{Eval}(g)) \subseteq \text{supp}(\text{Eval}(h))$.

The following two lemmas from the literature will be useful in the proof of Theorem \ref{thm:rmub}.
\begin{lemma}[\cite{abbe1}, Lemma 36]
	\label{lem:short}
	Let $\mathcal{V} \subseteq \mathbb{F}_2^m$ be such that $|\mathcal{V}|\geq 2^{m-u}$, for some $u\in \mathbb{N}$. Then, it holds that
	\[
	\text{rank}(G(m,r)[\mathcal{V}])> {m-u \choose \leq r},
	\]
	where $G(m,r)$ is the generator matrix of the RM$(m,r)$ code, and $G(m,r)[\mathcal{V}]$ denotes the set of columns of $G(m,r)$, indexed by $\mathcal{V}$.
\end{lemma}
The lemma below follows from Proposition~1.6 in \cite{sam}:
\begin{lemma}
	\label{lem:sam}
	Let $\{\mathcal{C}_n\}$ be a sequence of Reed-Muller codes of blocklength $n$, rate $R_n$, and  having weight distribution $\left(A_{\mathcal{C}_n}(w): 0\leq w\leq n\right)$. If $\lim_{n\to \infty} R_n = R$, then 
	\[
%	A_{\mathcal{C}_n}(w)\leq 2^{o(n)}\cdot\left(\frac{1}{1-R}\right)^{(2\ln2)w},
	A_{\mathcal{C}_n}(w) \leq 2^{o(n)} \cdot \exp_2\left(2 \cdot  \ln \biggl(\frac{1}{1-R}\biggr) \cdot w \right)
	\]
	where $o(n)$ denotes a term $a_n$ such that $\lim_{n\to \infty}\frac{a_n}{n} = 0$.
\end{lemma}
We now provide the proof of Theorem \ref{thm:rmub}.
\begin{proof}[Proof of Theorem~\ref{thm:rmub}]
	Fix the sequence $\{{\mathcal{C}}_m(R) = \text{RM}(m,r_m)\}$ of RM codes, with
	\[
		r_m = \max \left\{\left \lfloor \frac{m}{2}+\frac{\sqrt{m}}{2}Q^{-1}(1-R)\right \rfloor,0\right\},
	\]
	where $R\in (0,R^*)$, for $R^*$ as in the statement of the theorem.
	As explained in the discussion, any Boolean polynomial $f$ whose evaluation Eval$(f)\in {\mathcal{C}}_m$ can be expressed as
	\[
	f(x_1,\ldots,x_m) = g(x_1,\ldots,x_{m-1}) + x_m\cdot h(x_1,\ldots,x_{m-1}), 
	\]
	where $g,h$ are such that Eval$(g)\in \text{RM}(m-1,r)$ and Eval$(h)\in \text{RM}(m-1,r-1)$. Now, for any codeword Eval$(g) \in \text{RM}(m-1,r_m)$ of weight $w$, we shall first calculate the number, $N_w(g)$, of codewords Eval$(h) \in \text{RM}(m-1,r_m)$ such that supp$(\text{Eval}(g)) \subseteq \text{supp}(\text{Eval}(h))$. Note that $N_w(g)$ serves as an upper bound on the number of codewords Eval$(h) \in \text{RM}(m-1,r_m-1)$ such that the same property holds.
	
	To this end, suppose that for any weight $w$, the integer  $u=u(w)$ is the smallest integer such that wt$(\text{Eval}(g)) = w \geq2^{m-1-u}$. Note that for any polynomial $g$ as above of weight $w$, the number of codewords in the code produced by shortening RM$(m-1,r_m)$ at the indices in supp$(\text{Eval}(g))$ indeed equals $N_w(g)$. Now, since dim$(\text{RM}(m-1,r_m)) = {m-1\choose \leq r_m}$, and from the fact that $w\geq 2^{m-1-u}$, we obtain by an application of Lemma \ref{lem:short} and the rank-nullity theorem, that
	\begin{align}
		\label{eq:nw}
	N_w(g)&\leq \text{exp}_2\left({m-1\choose \leq r_m} - {m-1-u \choose \leq r_m}\right)\\
	&=:M_{u(w)}. \notag
	\end{align}
	%where the last equality holds since the upper bound on $N_w(g)$ depends on the polynomial $g$ only via a lower bound on its weight $w$. 
	
	Let $\mathsf{R}_{{\mathcal{C}},m}^{(1,\infty)}(R)$ be the rate of the largest $(1,\infty)$-subcode of ${\mathcal{C}}_m(R)$, i.e.,
	\[
	\mathsf{R}_{{\mathcal{C}},m}^{(1,\infty)}(R) = \frac{\log_2(|\mathcal{H}_{(1,\infty)}^{(m)}|)}{2^m},
	\]
	where we let $\mathcal{H}_{(1,\infty)}^{(m)}$ denote the largest $(1,\infty)$-subcode of ${\mathcal{C}}_m(R)$. Then, it holds that
	\begin{align}
|\mathcal{H}_{(1,\infty)}^{(m)}|&\leq \sum_{g: \text{Eval}(g)\in \text{RM}(m-1,r_m)}{N_w(g)} \notag	\\
		&\stackrel{(a)}{\leq} \sum\limits_{w=2^{m-1-r_m}}^{2^{m-1}}A_{m-1,r_m}(w){M_{u(w)}} \notag\\
		&\stackrel{(b)}{\leq} \left\{\sum\limits_{w=2^{m-1-r_m}}^{2^{m-2}}A(w){M_{u(w)}}\right\}+\frac{1}{2}\cdot \text{exp}_2\left(m-1\choose \leq r_m\right)\times \notag\\
		&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \ \text{exp}_2\left({m-1\choose \leq r_m} - {m-2\choose \leq r_{m}}\right)\notag \\
		&\stackrel{(c)}{\leq} \left\{\sum\limits_{w=2^{m-1-r_m}}^{2^{m-2}}A(w){M_{u(w)}}\right\}+
		\frac{1}{2}\times\notag\\
		&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \  \ \text{exp}_2\left({m-1\choose \leq r_m}+{m-2\choose \leq r_{m}}\right)\notag\\
		&\stackrel{(d)}{\leq} \Bigg\{\sum\limits_{i=1}^{{r_m-1}}A([2^{m-2-i}: 2^{m-1-i}])\times \notag\\
		&\ \ \ \ \ \ \ \ \ \ \ \   \text{exp}_2\left({m-1\choose \leq r_m} - {m-2-i \choose \leq r_m}\right)\Bigg\}+ \notag\\
		 &\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \frac{1}{2}\cdot\text{exp}_2\left({m-1\choose \leq r_m}+{m-2\choose \leq r_{m}}\right) \label{eq:sub1},
	\end{align}
where $A([a:b])$ is short for $\sum_{i=a}^{b}A(w)$. Here,
\begin{enumerate}[label = (\alph*)]
	\item follows from equation \eqref{eq:nw}, and
	\item holds due to the following fact: since the all-ones codeword $\mathbf{1}$ is present in RM$(m-1,r_m)$, it implies that $A_{m-1,r_m}(w) = A(w) = A(2^{m-1}-w)$, i.e., that the weight distribution of codewords is symmetric about weight $w=2^{m-2}$. Therefore,
	\begin{equation}
		\label{eq:Aw}
		A(w>2^{m-2})\leq \frac{1}{2}\cdot \text{exp}_2{m-1\choose \leq r_m}.
	\end{equation}
Next,
%	The strict inequality in (b) follows from the observation that the codeword Eval$(x_m)\in \text{RM}(m-1,r_m)$, for $m\geq 2$, and that wt$(\text{Eval}(x_m)) = 2^{m-2}$. 
	\item follows from Pascal's rule in combinatorics that for any $n,k \in \mathbb{N}$ with $n>k$:
	\[
	{n-1\choose k}+{n-1\choose k-1} = {n\choose k}.
	\]
	Picking $n=m-1$ and $k=r_m$, we obtain that
	\[
	{m-1\choose r_m}-{m-2\choose r_m} = {m-2\choose r_m-1},
	\]
	and hence that
	\[
	{m-1\choose \leq r_m}-{m-2\choose \leq r_m} < {m-2\choose \leq r_m}, \ \text{and}
	\]
	
	\item holds again from equation \eqref{eq:nw}.
\end{enumerate}
It is clear that a simplification of equation (d) depends crucially on good upper bounds on the weight distribution function. Now, since the code RM$(m-1,r_m)$ is obtained by shortening the code RM$(m,r_m)$ at positions $\mathbf{z} = (z_1,\ldots,z_m)$ where $z_m=1$, we obtain that $A_{m-1,r_m}(w)\leq A_{m,r_m}(w)$. 
%Note that the sequence of codes $\{{\mathcal{C}}_m(R) =\text{RM}(m,r_m)\}_{m\geq 1}$ is such that the sequence of dual codes $\{\text{RM}(m,m-r_m-1)\}_{m\geq 1}$ (see, for example, \cite{mws}) achieves a rate $1-R$ over the unconstrained BEC
Thus, we can use the result in Lemma \ref{lem:sam}, to get
\begin{align}
	&A_{m-1,r_m}([2^{m-2-i}: 2^{m-1-i}]) \notag\\
	&\leq A_{m,r_m}([2^{m-2-i}: 2^{m-1-i}]) \notag\\ 
	&\leq 2^{o(2^m)}\cdot \sum_{w=2^{m-2-i}}^{2^{m-1-i}}2^{2 \cdot \ln \left(\frac{1}{1-R}\right)\cdot w} \notag\\
	%&<  2^{o(2^m)}\cdot\sum_{w=2^{m-2-i}}^{2^{m-1-i}}2^{2\ln 2\cdot\log_2 \left(\frac{1}{1-R}\right)\cdot w} \notag\\
	%&<  \text{exp}_2\left(2\ln 2\cdot\log_2 \left(\frac{1}{1-R}\right)\cdot 2^{m-1-i}+o(2^m)\right) \notag\\
	&\leq 2^{o(2^m)}\cdot \text{exp}_2\left(2 \cdot \ln \left(\frac{1}{1-R}\right)\cdot 2^{m-1-i}\right) =: B_i(m) \label{eq:sub2}
\end{align}
Therefore, putting \eqref{eq:sub2} back in \eqref{eq:sub1}, we get that
\begin{align}
	&2^m\mathsf{R}^{(1,\infty)}_{{\mathcal{C}},m}(R)\notag \\
	& = \log_2|\mathcal{H}_{(1,\infty)}^{(m)}| \notag\\
	&\leq {m-1 \choose \leq r_m}+
	 \log_2\Bigg\{\frac{1}{2}\cdot \text{exp}_2{m-2 \choose \leq r_m}+\notag \\
	 &\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \sum_{i=1}^{r_m-1}B_i(m)\cdot \text{exp}_2\left( -{m-2-i \choose \leq r_m}\right)\Bigg\} \notag\\
	  &= {m-1 \choose \leq r_m}+\log_2\left(\alpha(m)+\beta(m)\right),\label{eq:subs3}
\end{align}
where we define
\begin{align}
	\alpha(m)&:= \frac12 \cdot \text{exp}_2{m-2 \choose \leq r_m}, \ \text{and} \notag\\
	\beta(m)&:= \sum_{i=1}^{r_m-1}B_i(m)\cdot \text{exp}_2\left( -{m-2-i \choose \leq r_m}\right). \label{eq:beta}
\end{align}
In Appendix A, we show that for all $\delta>0$ sufficiently small and for $m$ sufficiently large, it holds that
\begin{align}
\beta(m) \ & \le \ 2^{o(2^m)} \cdot \exp_2\Bigg( 2^{m-3}\Bigg[4\ln\left(\frac{1}{1-R}\right) - R(1-\delta)\Bigg]\Bigg) \notag \\ 
& =: \ \theta(m).
\label{eq:inter}
\end{align}
%Plugging the inequality above into \eqref{eq:subs3}, we see that
%\begin{align}
%2^m\mathsf{R}^{(1,\infty)}_{{\mathcal{C}},m}(R)\leq {m-1 \choose \leq r_m}+\log_2\left(\alpha(m)+\theta(m)\right).
%\label{eq:inter1}
%\end{align}
Now, using Lemma~\ref{lem:rate}, we have
\[
\lim_{m\to \infty} \frac{1}{2^m} {m-2 \choose \leq r_{m}} = \frac{R}{4}.
\]
Hence, for small $\delta>0$, and for $m$ large enough, it holds that
\[
{m-2 \choose \leq r_{m}}\leq (1+\delta)\cdot 2^{{m}-2}\cdot R.
\]
Therefore, we get that
\begin{align}
\alpha(m) \ \leq \ \text{exp}_2\left((1+\delta)\cdot2^{{m}-2}\cdot R\right) \ =: \ \eta(m). \label{eq:inter2}
\end{align}
Now, substituting \eqref{eq:inter} and \eqref{eq:inter2} in \eqref{eq:subs3}, we get that 
\begin{align}
2^m\mathsf{R}^{(1,\infty)}_{{\mathcal{C}},m}(R)\leq {m-1 \choose \leq r_m}+\log_2\left(\eta(m)+\theta(m)\right).
\label{eq:inter3}
\end{align}
Putting everything together, we see that
\begin{align}
	&{R}^{(1,\infty)}_{{\mathcal{C}}}(R) \notag\\ &= \limsup_{m\to \infty}\mathsf{R}^{(1,\infty)}_{{\mathcal{C}},m}(R)\notag\\
	&\leq \lim_{m\to \infty} \frac{1}{2^m} \left[{m-1 \choose \leq r_m}+\log_2\left(\eta(m)+\theta(m)\right)\right] \notag\\
	&\stackrel{(a)}{\leq} \lim_{m\to \infty} \frac{1}{2^m} \left[{m-1 \choose \leq r_m}+\log_2\left(2\cdot \theta(m)\right)\right] \notag\\
	&\stackrel{(b)} =\frac{R}{2} + \lim_{m\to \infty} \frac{1}{2^m} \cdot \log_2 \theta(m) \notag \\
%	&\stackrel{(b)} =\frac{R}{2} + \lim_{m\to \infty} \frac{1}{2^m}\log_2\Bigg\{(r_m-1)\cdot\text{exp}_2\Bigg( 2^{m-3}\Bigg[4\ln \Bigl(\frac{1}{1-R}\Bigr) - R(1-\delta)  \notag\\
%	& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \log_2 \left(\frac{1}{1-R}\right) - R(1-\delta)\Bigg]+o(2^m)\Bigg)\Bigg\}\notag\\
	&= \frac{R}{2}+\frac{4  \ln\left(\frac{1}{1-R}\right)  - 
		R(1-\delta)}{8} \notag\\
	&= \frac{3R}{8}+\frac{1}{2}\ln \left(\frac{1}{1-R}\right)+\frac{R\delta}{8} \label{eq:final}.
\end{align}
Note that inequality (a) follows from the fact for any $R \in (0,1)$, $\eta(m)\leq \theta(m)$ holds for all sufficiently small $\delta > 0$. Further, equation (b) is valid because $\lim_{m\to \infty} \frac{1}{2^m} {m-1 \choose \leq r_m} = \frac{R}{2}$, by Lemma~\ref{lem:rate}. Since equation \eqref{eq:final} holds for all $\delta>0$ sufficiently small, we can let $\delta\to 0$, thereby obtaining that
\begin{align}
	\label{eq:finalf}
	{R}^{(1,\infty)}_{{\mathcal{C}}}(R) \le \frac{3R}{8}+\frac{1}{2}\ln \left(\frac{1}{1-R}\right).
\end{align}
It can be numerically verified that for $R\in (0,R^*)$, where $R^*$ is as in the statement of the theorem, it holds that the right-hand side of equation \eqref{eq:finalf} is less than $R$, thereby providing a non-trivial upper bound. Finally, we note that since $|\mathcal{H}_{(1,\infty)}^{(m)}|\leq |\mathcal{C}_m(R)|$, the trivial upper bound of ${R}^{(1,\infty)}_{{\mathcal{C}}}(R)\leq R$ holds for all $R\in (0,1)$.
%\textbf{\textbackslash end}
\end{proof}



%\textbf{\textbackslash end}

%\begin{align}
%	\mathsf{R}_{(1,\infty)}^{\text{RM}} &= \lim_{m\to \infty} \mathscr{R}_{(1,\infty)}^{(m)} \notag\\
%	&< \lim_{m\to \infty} \frac{{m-1 \choose \leq v_m}+{m-2\choose \leq v_m}}{2^m} \notag\\
%	&= \frac{3R}{4}, \label{eq:append}
%\end{align}
%where the proof of equation \eqref{eq:append} is postponed to Appendix B. The proof follows along similar lines as the last part of the proof of Theorem \ref{thm:rm}, but crucially employs the assumption that $R<0.5$. Since the arguments must hold for any capacity-achieving (over the unconstrained BEC) sequence of RM codes, a more careful bounding technique is required.
%\end{proof}
%
%Note that we have only as yet proved an upper bound for the special case when $d=1$. However, before we generalize the arguments to all $d$, it is important that we analyze the consequences of Theorem \ref{thm:rmub}. Indeed, it is true that for any $\epsilon \in (0.5,1)$,
%\begin{equation}
%	\label{eq:rmubeps}
%	\mathsf{R}_{(1,\infty)}^{\text{RM}}<\frac{3}{4}(1-\epsilon).
%\end{equation}
%\begin{figure*}[!t]
%	\centering
%	
%	\includegraphics[width=0.9\textwidth]{RMub_achMarkov.png}
%	\caption{Figure shows a comparison between the best numerical information rate achieved using stationary, ergodic first-order Markov input distributions, and the upper bound provided in equation \eqref{eq:rmubeps}, for $\epsilon>0.5$.}
%	\label{fig:rmub}
%\end{figure*}
%Figure \ref{fig:rmub} shows a comparison between the upper bound in equation \eqref{eq:rmubeps}, on the rate achieved by using $(1,\infty)$-RLL subcodes of any capacity-achieving (over the unconstrained BEC) sequence of RM codes, and numerical lower bounds on the capacity without feedback of the $(1,\infty)$-RLL input-constrained BEC. These lower bounds are computed using numerical sampling-based algorithms (see, for example, \cite{Arnold} or \cite{arnk21ncc}), which consider stationary, ergodic, first-order Markov input distributions, and compute their information rates. It is clear from the plots that the upper bound in equation \eqref{eq:rmubeps} is less than the achievable rates of Markov input processes, for $\epsilon>0.5$. Therefore, we conclude that it is not possible to achieve the capacity of the $(1,\infty)$-RLL input-constrained BEC by using $(1,\infty)$-RLL subcodes of RM codes under the lexicographic ordering.
%\begin{remark}
%	While we have proved a pessimistic result under the lexicographic ordering of co-ordinates of the RM code, it is unclear what the best achievable rates are of $(1,\infty)$-RLL subcodes of RM codes obtained by permuting co-ordinates.
%\end{remark}
%We now extend the proof of Theorem \ref{thm:rmub} to general $d$. For ease of notation, we let $z := \left \lceil \log_2(d+1)\right \rceil$. Similar to equation \eqref{eq:rmdecomp}, we note that for any $f\in \mathbb{F}_2[x_1,\ldots,x_m]$, with Eval$(f) \in \text{RM}(m,r)$, it is true that:
%\begin{align}
%	\label{eq:genddecomp}
%f(x_1,\ldots,x_m) &= g_0(x_1,\ldots,x_{m-z})+\notag\\ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \ \  &\sum_{\substack{{S\subseteq [m-z+1:m],}\\{\ S\neq \emptyset}}} x_Sg_S(x_1,\ldots,x_{m-z}),
%\end{align}
%where we use the notation $x_S$ to denote the monomial $\prod_{i\in S}x_i$, and $g_0$ is such that Eval$(g_0)\in \text{RM}(m-z,r)$ and for any nonempty $S\subseteq [m-z+1:m]$, the polynomials $g_S$ are such that Eval$(g_S)\in \text{RM}(m-z,r-|S|)$.
%
%An important ingredient in the proof for general $d$ is the following lemma, which is a generalization of Lemma \ref{lem:necesscond}:
%\begin{lemma}
%	\label{lem:gend}
%	If a codeword Eval$(f)\in \text{RM}(m,r)$ respects the $(d,\infty)$-RLL constraint, then, supp$(Eval(g_0))\subseteq \text{supp}(\text{Eval}(g_S))$, for all polynomials $g_S$, where $S\subseteq [m-z+1:m]$ is non-empty, and $g_0$ and $g_S$ are as in \eqref{eq:genddecomp}.
%\end{lemma}
%\begin{proof}
%	To this end, we need to show that for any $\mathbf{z}\in \mathbb{F}_2^{m-z}$, it must be that $g_S(\mathbf{z}) = 1$, for all non-empty subsets $S\subseteq [m-z+1:m]$, whenever $g_0(\mathbf{z})=1$, in order for Eval$(f)$ to respect the $(d,\infty)$-RLL constraint. This follows from the simple observation that the Boolean polynomial $\theta(x_{m-z+1},\ldots,x_m):=\prod_{S\subseteq [m-z+1:m]} x_S$ is the only polynomial in the $\left \lceil \log_2(d+1)\right \rceil$ variables $x_{m-z+1},\ldots,x_m$, with the property that $\theta(\mathbf{0}) = 1$ and $\theta(\mathbf{z}) = 0$, for all $\mathbf{z}\neq \mathbf{0}$.
%\end{proof}
%With the lemma above in place, the remainder of the proof of Theorem \ref{thm:rmub} for general $d$ follows similar to the proof when $d=1$. Some salient features are described in the proof below:
%\begin{proof}
%	As earlier, we work with a capacity-achieving (over the unconstrained BEC) sequence of RM codes, $\{\hat{\mathcal{C}}_m = \text{RM}(m,v_m)\}$. 
%	
%	We let $N_w^{(d)}(g_0)$ denote the number of codewords, Eval$(g_S) \in \text{RM}(m-z,r-|S|)$, for non-empty subsets $S\subset [m-z+1:m]$, such that supp$(\text{Eval}(g_0))\subseteq \text{supp}(\text{Eval}(g_S))$, for all $g_S$. We then obtain, similar to equation \eqref{eq:nw}, that:
%	\[
%	N_w^{(d)}(g_0)\leq \text{exp}_2\left((2^z-1)\cdot\left({m-z\choose \leq v_m} - {m-z-u \choose \leq v_m}\right)\right),
%	\]
%	when wt$(\text{Eval}(g_0))\geq 2^{m-z-u}$. Also, we define $\mathscr{R}_{(d,\infty)}^{(m)}$ to be the rate of any $(d,\infty)$-subcode of $\hat{\mathcal{C}}_m$, i.e.,
%	\[
%	\mathscr{R}_{(d,\infty)}^{(m)} = \frac{\log_2(|\mathcal{H}_{(d,\infty)}^{(m)}|)}{2^m},
%	\]
%	where we let $\mathcal{H}_{(d,\infty)}^{(m)}$ denote a $(d,\infty)$-subcode of $\hat{\mathcal{C}}_m$. For ease of reading, we let $\alpha_m^{(d)}:= |\mathcal{H}_{(d,\infty)}^{(m)}|$. Equations \eqref{eq:sub1} and \eqref{eq:sub2} can then be modified to take into account the fact that Eval$(g_0) \in \text{RM}(m-z, v_m)$, and we finally get that:
%	\begin{align}
%		\mathsf{R}_{(d,\infty)}^{\text{RM}} &= \lim_{m\to \infty} \mathscr{R}_{(d,\infty)}^{(m)} \notag\\
%		&< \lim_{m\to \infty} \frac{{m-z \choose \leq v_m}+(2^z-1){m-z-1\choose \leq v_m}}{2^m} \notag\\
%		&= R\cdot \left(\frac{2^z+1}{2^{z+1}}\right), \label{eq:gendappend}
%	\end{align}
%where the complete proof of the equality in \eqref{eq:gendappend} follows from the treatment in Appendix B.
%\end{proof}
